Auto-FP: An Experimental Study of Automated Feature Preprocessing for Tabular Data

Classical machine learning models, such as linear models and tree-based models, are widely used in industry. These models are sensitive to data distribution, thus feature preprocessing, which transforms features from one distribution to another, is a crucial step to ensure good model quality. Manually constructing a feature preprocessing pipeline is challenging because data scientists need to make difficult decisions about which preprocessors to select and in which order to compose them. In this paper, we study how to automate feature preprocessing (Auto-FP) for tabular data. Due to the large search space, a brute-force solution is prohibitively expensive. To address this challenge, we interestingly observe that Auto-FP can be modelled as either a hyperparameter optimization (HPO) or a neural architecture search (NAS) problem. This observation enables us to extend a variety of HPO and NAS algorithms to solve the Auto-FP problem. We conduct a comprehensive evaluation and analysis of 15 algorithms on 45 public ML datasets. Overall, evolution-based algorithms show the leading average ranking. Surprisingly, the random search turns out to be a strong baseline. Many surrogate-model-based and bandit-based search algorithms, which achieve good performance for HPO and NAS, do not outperform random search for Auto-FP. We analyze the reasons for our findings and conduct a bottleneck analysis to identify the opportunities to improve these algorithms. Furthermore, we explore how to extend Auto-FP to support parameter search and compare two ways to achieve this goal. In the end, we evaluate Auto-FP in an AutoML context and discuss the limitations of popular AutoML tools. To the best of our knowledge, this is the first study on automated feature preprocessing. We hope our work can inspire researchers to develop new algorithms tailored for Auto-FP.

==> src/auto-feat.tex <==
\vspace{-.25em}
\section{Automated Feature Preprocessing}

Scikit-learn \cite{scikit-learn} is a widely used ML tool and it is especially good at handling structure data. It contains a feature preprocessing module with many preprocessors\footnote{https://scikit-learn.org/stable/modules/preprocessing.html}. In this section, we first introduce these feature preprocessors. Then we explore whether feature preprocessing really matters and motivate the Auto-FP problem. Thirdly, we define the Auto-FP problem. Finally, we discuss the relationship of Auto-FP with HPO and NAS.



%Feature preprocessing with single preprocessor is popular in \texttt{Kaggle} and \texttt{OpenML}. However, not many works try to investigate whether combining multi-preprocessors as a pipeline is a better solution or not. In this section, firstly, we introduce the 7 commonly used feature preprocessors. Secondly, we explore whether combining these feature preprocessors as pipelines can improve the performance of ML model and emphasize the importance of feature preprocessing automation. Finally, we give the explicit formulation of automatic feature preprocessing problem.
\subsection{Feature Preprocessors}
\label{operator}


\begin{figure}[t] 
% \vspace{-1.5em}
\centering 
\includegraphics[width=1.0\linewidth]{figures/preprocessors_example.pdf}
\vspace{-2em}
\caption{Illustration of different feature preprocessors. (a) No preprocessor; (b) Binarizer; (c) MaxAbsScaler; (d) MinMaxScaler; (e) Normalizer; (f) PowerTransformer; (g) QuantileTransformer; (h) StandardScaler.} 
\label{fig:preprocessors_example} %\vspace{-1em}
\end{figure}



We introduce commonly used feature preprocessors in Scikit-learn~\cite{scikit-learn}. % Figure \ref{fig:preprocessors_example} shows the example calculation results of the seven preprocessors. Note that Figure \ref{fig:preprocessors_example}(a) is the origin data column without any preprocessing.

%\jn{Is it possible to add a figure and use it to show how the same column will be transformed to after applying each preprocessor?} \Danrui{Added.}


\textbf{1.\textit{Binarizer: }} \textit{Binarizer} binarizes data into two values (0 or 1) according to a threshold. Values greater than the threshold are mapped to 1, otherwise to 0. The default threshold is 0, which means that negative values are mapped to 0, non-negative values are mapped to 1. E.g., Figure~\ref{fig:preprocessors_example}(a) is the original feature without any preprocessing. Figure~\ref{fig:preprocessors_example}(b) shows the result of applying \textit{Binarizer} to the feature. With the default threshold 0, the number -1.5 is transformed to 0, while the other values are transformed to 1. 

\textbf{2. \textit{MaxAbsScaler: }} \textit{MaxAbsScaler} scales each feature according to its maximum absolute value. Let $x$ be the maximum absolute value of the feature. For each value $v_1, v_2, \cdots$ of the feature, the scaled values will be $\frac{v_1 }{x}, \frac{v_2}{x}, \cdots$. Figure \ref{fig:preprocessors_example}(c) shows the result of applying \textit{MaxAbsScaler} to the original feature. The maximum absolute value of the original feature is 5. Thus, the value -1.5 is transformed to $\frac{-1.5}{5} = -0.3$ and the value 4 is transformed to $\frac{4}{5} =0.8$.

\textbf{3. \textit{MinMaxScaler: }}  \textit{MinMaxScaler} transforms features by scaling each feature to a given range ([0, 1] by default).  Let $\max$ and $\min$ denote the maximum and minimum value of the feature, respectively. The scaled result of $x$ is calculated as $\frac{x - min}{max - min}$. Figure \ref{fig:preprocessors_example}(d) shows the result of applying \textit{MinMaxScaler} to the original feature. The max (min) value of the original feature is 5 (-1.5).  Thus, the value 1 is transformed to $\frac{1-(-1.5)}{5-(-1.5)}=0.38$.

\textbf{4. \textit{Normalizer: }} \textit{Normalizer} normalizes samples (\emph{rows} of data) individually into unit norm. Given a row vector, $x = [x_1, x_2, \cdots, x_n]$, each value $x_i$ is scaled to $\frac{x_i}{||x||_{2}}$, where $||x||_{2} = \sqrt{\sum_{i = 1}^{n} x_i^2}$ is the Euclidean length of the row vector. Suppose the data only has a single column as shown in Figure~\ref{fig:preprocessors_example}(a). Figure~\ref{fig:preprocessors_example}(e) shows the result of applying \textit{Normalizer} to the data. For the first row $x = [-1.5]$, the Euclidean length is $||x||_{2} = \sqrt{(-1.5)^2} = 1.5$, thus the value -1.5 is transformed to $\frac{-1.5}{1.5}=-1$.


%, which means the normalization process for each sample is independent.  \texttt{Scikit-Learn} \cite{scikit-learn} library gives three choices of normalizing way, which are \textit{L1, L2} and \textit{Max}. The \textit{L2} way is the default way in \texttt{Scikit-Learn} \cite{scikit-learn} library. In this paper, we also employ the default \textit{L2} way for \textit{Normalizer}, \jn{Which way did we use? Let's only describe the way we use and justify why we use it.} \Danrui{We use L2 way because Sklearn uses L2 as the default way, I just delete the description of L1 and Max ways.}
%The \textit{L1} way calculates the Manhanttan Distance of each sample. Thus, the normalization factor $z_{1}$ of \textit{L1} way is calculated by Eq. \ref{eq:z1}. The \textit{L2} way 
%which considers the Euclidean Distance of each feature. The normalization factor $z$ of \textit{L2} way is calculated by Eq. \ref{eq:z2}. 
%The \textit{Max} way considers the maximum value of each sample as the normalization factor, as Eq. \ref{eq:zmax} shows. 
%The final normalization results are calculated by each value of each sample dividing its normalization factor. Figure \ref{fig:preprocessors_example}(e) shows the result of applying \textit{Normalizer} on column \texttt{Num}. The normalization factor of the first row of column \texttt{Num} is $\sqrt{(-1.5)^2} = 1.5$, thus the transformed result of value -1.5 is (-1.5)/1.5=-1.
%    \begin{equation}
%    \label{eq:z1}
%        z_{1} = ||x||_{1} = \sum_{i = 1}^{n} |x_i|
%    \end{equation}
    
    %\begin{equation}
   % \label{eq:z2}
   %     z = ||x||_{2} = \sqrt{\sum_{i = 1}^{n} x_i^2}
   % \end{equation}
    
%    \begin{equation}
%    \label{eq:zmax}
%        z_{max} = max\{x_i\}
%    \end{equation}
    
\textbf{5. \textit{PowerTransformer: }} \textit{PowerTransformer} applies an exponential transformation to each feature to make its distribution more normal-like. It can help ML models with normal-like input assumption and help to handle very skew data. The default PowerTransformer of Scikit-Learn, called Yeo-Johnson transformation, is defined as follows:
\begin{equation}
    \label{yeo-johnson}
    Yeo-Johnson(x) = 
        \begin{cases}
        \frac{(x+1)^{\lambda} - 1}{\lambda}& x >= 0, \lambda \neq 0\\
        log(x + 1) & x >= 0, \lambda = 0 \\
        \frac{1 - (1 - x)^{2 - \lambda}}{2 - \lambda} & x < 0, \lambda \neq 2 \\
        -log(1 - x) & x < 0, \lambda = 2
        \end{cases}
    \end{equation}
where $\lambda$ is automatically calculated. It aims to fit the transformed feature into a zero-mean, unit-variance normal distribution as much as possible. Figure \ref{fig:preprocessors_example}(f) shows the result of applying \textit{PowerTransformer} to the original feature. At first, the \textit{PowerTransformer} finds the optimal $\lambda$ automatically, which is 1.22. Then, the transformed results are calculated by Equation~\ref{yeo-johnson}. For example, the transformed result of value -1.5 is $\frac{1-(1-(-1.5))^{2-1.22}}{2-1.22}=-1.34$. %With Equation \ref{yeo-johnson}, the transformed results of \texttt{Num} is $[-1.34, 1.09, 1.69, 2.96, 3.63, 5.02, 6.47]^T$. Note that by default, the \textit{PowerTransformer} enables the standardizing option. Thus the final result is the standardized version of previous transformation vector.

%\jn{Similar to my above comment, which transformation did we use? what's the default $\lambda$?} \Danrui{We use the default Yeo-johnson. And there is no default labmda, labmda is calculated for each column when calling PowerTransformer, I add these content in the following text .}\texttt{Scikit-Learn} provides 
%the Box-Cox transformation (Equation \ref{box_cox}) and 
%the default Yeo-Johnson transformation (Equation \ref{yeo-johnson}). 
%The Box-Cox transformation requires input data to be strictly positive, while the Yeo-Johnson transformation 
%which supports both positive and negative data. We also utilize Yeo-Johnson transformation by default in our paper. Notice that there is an important parameter $\lambda$ which is deterministic. $\lambda$ controls the quality of approximation of a normal distribution curve, which means that the best $\lambda$ makes the transformed distribution be nearest with a normal distribution.  \jn{Why is it in red?} \Danrui{Re-ensured in Sklearn document, the step of lambda is used to transform column into normal distribution, then standardize the whole column.}\texttt{Scikit-Learn} library optimizes $\lambda$ while calculating transformation results. Then \texttt{Scikit-Learn} uses default parameter $standardize = True$ to transform results generated by $\lambda$ to a zero-mean, unit-variance normal distribution. 

%Figure \ref{fig:preprocessors_example}(g) shows the result of applying \textit{PowerTransformer} on column \texttt{Num}. At first, the \textit{PowerTransformer} find the optimal $\labmda$ automatically, which is 1.22. Then, the transformed results are calculated by Equation \ref{yeo-johnson}. For example, the transformed result of value -1.5 is $\frac{1-(1-(-1.5))^{2-1.22}}{2-1.22}=-1.34$. With Equation \ref{yeo-johnson}, the transformed results of \texttt{Num} is $[-1.34, 1.09, 1.69, 2.96, 3.63, 5.02, 6.47]^T$. Note that by default, the \textit{PowerTransformer} enables the standardizing option. Thus the final result is the standardized version of previous transformation vector.
    %\begin{equation}
    %\label{box_cox}
    %Box-Cox(x) = 
    %    \begin{cases}
    %    \frac{x^{\lambda} - 1}{\lambda}& \lambda \neq 0\\
    %    log(x) & \lambda = 0
    %    \end{cases}
    %\end{equation}
  \iffalse  
    \begin{equation}
    \label{yeo-johnson}
    Yeo-Johnson(x) = 
        \begin{cases}
        \frac{(x+1)^{\lambda} - 1}{\lambda}& x >= 0, \lambda \neq 0\\
        log(x + 1) & x >= 0, \lambda = 0 \\
        \frac{1 - (1 - x)^{2 - \lambda}}{2 - \lambda} & x < 0, \lambda \neq 2 \\
        -log(1 - x) & x < 0, \lambda = 2
        \end{cases}
    \end{equation}
    \fi
 
\textbf{6. \textit{QuantileTransformer: }} \textit{QuantileTransformer} transforms features independently into a uniform or a normal distribution. Since the above PowerTransformer can be used for normal distribution, we utilize QuantileTransformer for uniform distribution. Intuitively, each transformed value represents its quantile position in the original feature column. For example, Figure~\ref{fig:preprocessors_example}(a) shows the original feature column: [-1.5, 1, 1.5, 2.5, 3, 4, 5]. As shown in Figure~\ref{fig:preprocessors_example}(g), it is transformed to  $[\frac{0}{6}, \frac{1}{6}, \frac{2}{6}, \frac{3}{6}, \frac{4}{6}, \frac{5}{6}, \frac{6}{6}]  = [0, 0.17, 0.33, 0.5, 0.67, 0.83, 1]$. 

\iffalse

\jn{Why is it in red?} \Danrui{because we don't use normal distribution in out paper} distribution. In this paper, we use the default setting in \texttt{Scikit-Learn} of transforming into uniform distribution. This transformation include two steps: (1) calculate the reference values and the actual quantile values according to input data column and number of quantiles (2) estimate transformed data according to the actual quantile values and the reference values. 

Figure \ref{fig:preprocessors_example}(g) shows the result of applying \textit{QuantileTransformer} on column \texttt{Num}. With the default setting, the number of quantiles is 1000. However, when the number of data rows is smaller than 1000, the number of quantiles will be set to the number of data rows automatically. Thus, the number of quantiles of column \texttt{Num} is 7. At first, we can calculate that the reference values are $ref = [0, 0.17, 0.33, 0.5, 0.67, 0.83, 1]$. According to these reference values, we know that 0 in $ref$ is corresponding to the minimal value -1.5 in \texttt{Num}, and 1 in $ref$ is corresponding to the maximal value 5 in \texttt{Num}. Then we need to calculate what values that 1 and 1.5 are corresponding to. We notice that there are in total 6 gaps in \texttt{Num} with 7 numbers, thus each gap get (1-0)/5=0.17. As for the reference value 0.17, it takes 0.17/0.17 = 1 gaps, which means that the value 0.17 is corresponding to is in the second row of \texttt{Num}, which is 1. With the same way, we get the corresponding values of $ref$ is just column \texttt{Num}. In the second step, we map a function between $quan$ and $ref$. The $quan$ is the list of X-values and $ref$ is the list of Y-values. Obviously it is a 1-to-1 map. Thus finally we get transformed column of \texttt{Num}, which is shown in Figure \ref{fig:preprocessors_example}(g).  
%For example, if there is a list of numbers $a = [1, 1.5, 2.5, 3, 4, 5]$ and a number of quantiles 4, at first, we can calculate that the reference values are $ref = [0, 0.33, 0.67, 1]$. According to these reference values, we know that 0 in $ref$ is corresponding to the minimal value 1 in $a$, and 1 in $ref$ is corresponding to the maximal value 5 in $a$. Thus we need to calculate what values 0.33 and 0.67 is corresponding to. We notice that there are in total 5 gaps in $a$ with 6 numbers, thus each gap get (1-0)/5=0.2. As for the reference value 0.33, it takes 0.33/0.2 = 1.65 gaps, which means that the value 0.33 is corresponding to is between 1.5 and 2.5. The gap between 1 and 1.5 is counted as 1 gap, and we should calculate the remaining 0.65 gap between 1.5 and 2.5. Thus, the estimated 0.33 quantile value is $1.5 + (2.5 - 1.5) \times 0.65 = 2.15$. In the same way, the estimated 0.66 quantile value is $3 + (4 - 3) \times 0.3 = 3.3$. Finally, we get the reference values of $ref = [0, 0.33, 0.67, 1]$ and their corresponding quantile values $quan = [1, 2.15, 3.3, 5]$.

%In the second step, we map a function between $quan$ and $ref$. The $quan$ is the list of X-values and $ref$ is the list of Y-values. Rethinking each value in $a$ again: 1 is corresponding to 0, 5 is corresponding to 1. As for 1.5 which is between 1 and 2.15, we use linear interpolation to calculate the transformed value, which is $0+\frac{1.5-1}{2.15-1} \times (0.33-0) = 0.14$. With the same way, finally we get transformed column of $a$, which is [0, 0.14, 0.43, 0.57, 0.8, 1].  
\jn{Explain why it multiplies 0.2? I did not quite get this part.} \Danrui{I rewrite this part. Now you can re-read it to see if you can get the main idea of calculation through the new example.}
%For example, if there is a list of numbers [1, 1.5, 2.5, 3, 5] and the 30 percent quantile need to be calculated, we firstly get the number $1 + (5-1) \times 0.3 = 2.2$ to indicate the position should be between [1.5, 2.5] (the second and third position in the number list). Then the fraction stands for the linear incorporation fraction. Finally, the 30 percent quantile should be $1.5 + (2.5 - 1.5) \times 0.2 = 1.7$. 
%It can reduce the distance between (marginal) outliers and normal values.

\fi
    
\textbf{7. \textit{StandardScaler: }} \textit{StandardScaler} standardizes the feature according to its mean value and standard deviation. Let $\mu$ and $\sigma$ denote the mean and standard deviation of the feature column. For each value $x$ in the feature column, the scaled result  is calculated by $\frac{x - \mu}{\sigma}$. Figure \ref{fig:preprocessors_example}(h) shows the result of applying \textit{StandardScaler}. The $\mu$ and $\sigma$ of column \texttt{Num} are 2.21 and 1.98.  Thus, the transformed result of value -1.5 is $\frac{-1.5-2.21}{1.98} =-1.87$. 
%\jn{I change 2.2143 to 2.21 and 1.9794 to 1.98. Please update the values in Figure \ref{fig:preprocessors_example}(h) } \Danrui{Updated.}

\stitle{Remark.} Our work considers a total of seven widely used preprocessors, which is more than what AutoML tools support (see Section~\ref{sec:automl} for more detail). Hence, the findings derived from this paper are applicable to a wide range of scenarios. For the situations when more preprocessors are needed, one can easily extend our benchmark to derive additional insights. 



%\subsection{Feature Preprocessing Pipelines}

%\subsection{Automatic Feature Preprocessing}

%\paragraph{The Workflow}
%\begin{figure}[htbp] % picture
%    \centering
%    \includegraphics[width=0.9\linewidth]{workflow.pdf}
%    \caption{Workflow overview of automated feature preprocessing.}
%    \label{fig:workflow}
%\end{figure}

%The high-level workflow of automated feature preprocessing is shown in Figure \ref{fig:workflow}. Training data and validation data are derived from different data sources, integrated by entity matching and cleaned by cleaning algorithms. After inputting the training data into automated feature preprocessing process, the process aims to find preprocessing pipeline with best validation score. Thus, it processes training data with pipeline and trains the downstream ML model. Validation data is needed to get validation score of ML model. Validation score is considered as feedback of automated feature preprocessing. If the score is not good enough, the process continues finding next preprocessing pipeline, until achieving the iteration or time limit.

\subsection{Does Feature Preprocessing Really Matter?}
To motivate Auto-FP, we conduct an exploratory experiment to examine whether feature preprocessing really matters.

Since it is expensive to enumerate all possible pipelines, we only consider pipelines whose length is no larger than 4, leading to a total of 2800 different pipelines. For each pipeline, we apply it to a training set and then train a LR model on the preprocessed dataset. We plot the distribution of model accuracy of 2800 pipelines. Figure~\ref{fig:order_impact} shows the results on four benchmark datasets (the description of these datasets can be found in Section~\ref{exp-setup}).  The x-axis represents different model accuracy values; the y-axis represents how many pipelines can achieve the accuracy. The red line indicates the ML accuracy without any preprocessing. 

We can see that different pipelines lead to significantly different model accuracy. For example, on the Heart dataset in Figure~\ref{fig:order_impact}, the model accuracy is spread out from 0.49 to 0.88. 
%\jn{Replace 0.48 and 0.84 with the actual values}. \Danrui{Replaced}
Furthermore, a good pipeline can significantly improve the model accuracy. For example, as shown in Figure~\ref{fig:order_impact}, the model accuracy of the best pipeline on \textit{Pd} dataset is 0.94, while no pipeline (i.e., the red line) can only achieve an accuracy of 0.81. These results validate the importance of feature preprocessing. 
%\jn{please update 0.92 and 0.8  with the actual values } \Danrui{Replaced.}

%In general, with proper number of operators and proper order, the best feature preprocessing pipeline in 2800 pipelines can significantly improve the validation accuracy of downstream ML model, which means that (1) the performance of downstream ML model like Logistic Regression can indeed be improved by feature preprocessing (2) constructing multi-preprocessors into a feature preprocessing pipeline is really meaningful. %\textcolor{red}{Analyze the difference between different ML models.}  


%In this section, we investigate the effectiveness of operator's number and order. We use 7 preprocessors in \texttt{Scikit-Learn} \cite{scikit-learn} library listed in Section 2.1. 

%\subsection{The effectiveness of operator's number and order}
%We test the 10 datasets with feature preprocessing pipelines of which max length is 4. The number of feature preprocessing pipelines in this small experiment is 2800. We set the downstream ML model as Logistic Regression. Then we generate distribution of validation accuracy in Figure \ref{fig:order_impact}. The red line means the ML accuracy without any change. The X-axis means the accuracy of ML model, and the Y-axis means how many pipelines can achieve the accuracy.

%\begin{figure}[t]
%\centering
%\subfigure[Australian]{
%\label{Fig.sub.1}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_austrilian_LR.eps}}
%\subfigure[Blood]{
%\label{Fig.sub.2}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_blood_LR.eps}}
%\subfigure[Emotion]{
%\label{Fig.sub.3}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_emotion_LR.eps}}
%\subfigure[Heart]{
%\label{Fig.sub.4}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_heart_LR.eps}}
%\subfigure[Forex]{
%\label{Fig.sub.5}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_forex_LR.eps}}
%\subfigure[Jasmine]{
%\label{Fig.sub.6}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_jasmine_LR.eps}}
%\subfigure[Madeline]{
%\label{Fig.sub.7}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_madeline_LR.eps}}
%\subfigure[Pd\_speech\_features]{
%\label{Fig.sub.8}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_pd_LR.eps}}
%\subfigure[Wine\_quality]{
%\label{Fig.sub.9}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_wine_LR.eps}}
%\subfigure[Thyroid\_allhyper]{
%\label{Fig.sub.10}
%\includegraphics[width=0.22\textwidth]{figures/order_impact_thyroid-allhyper_LR.eps}}
%\caption{Distribution of LR accuracy under different feature preprocessing pipelines. 
%\jn{update dataset names with short names; change ``no prep'' to ``no FP'' }\Danrui{Updated}
%} 
%\label{fig:order_impact}
%\end{figure}

\begin{figure}[t]
% \vspace{-3em}
\vspace{-1.5em}
\centering
\includegraphics[width=\columnwidth]{figures/order_impact_all_in_one.eps}
\vspace{-2em}
\caption{Distribution of LR accuracy under different feature preprocessing pipelines.
}
\label{fig:order_impact}
\end{figure}


%Designing "good" feature preprocessing pipelines according to datasets and downstreamin ML model is a very tedious and time-consuming task, which need the knowledge of experts and tries over and over again by human in practice. That is the motivation for us to automating the finding process of feature preprocessing pipelines for specific data and dwonstreaming ML model. 

\iffalse

\jn{Are we able to get the following conclusion from Fig 1?} \Danrui{Actually not very obvious, thus I deleted the conclusion and changed to another expression.} Note that in Figure \ref{fig:order_impact}, after we enumerate and evaluate all 2800 pipelines, we can figure out what the best pipeline is, which is a process with lots effort. Although the 2800 pipelines and downstream ML model are same, the accuracy distributions of these pipelines are still quite different on different datasets, which means that different datasets will cause the same pipeline gives different accuracy results. This conclusion can be also derived from Table \ref{tab:acc_order_impact_same_model}. For instance, the performance of the feature preprocessing pipeline with \textit{QuantileTransformer} varies a lot on different datasets. 

%Also, the number and order of feature preprocessors significantly affect the final validation accuracy, which is illustrated well in \ref{fig:order_impact}.  For example, with different lengths and orders of feature preprocessors, the performance of LR on \textit{Wine\_quality} dataset shows different values. The minimal validation accuracy is approximate to zero and the maximal is approximate to 0.6. 
\begin{table}[t]% h asks to places the floating element [h]ere.
  \caption{The accuracy of applying preprocessors on different datasets with LR model.}
  \label{tab:acc_order_impact_same_model}
  \small
  \begin{tabular}{p{0.27\linewidth}<{\centering}
                  p{0.1\linewidth}<{\centering}
                  p{0.1\linewidth}<{\centering}
                  p{0.16\linewidth}<{\centering}
                  p{0.16\linewidth}<{\centering}}
    \toprule
    \textbf{Preprocessor} & \textbf{Heart} & \textbf{Forex} & \textbf{\makecell{Pd\_speech\\ \_features}} & \textbf{\makecell{Wine\\ \_quality}}\\ 
    \midrule
    Binarizer           & 0.6326 & 0.5173 & 0.7933 & 0.4375\\ 
    Standardizer        & 0.7755 & 0.5928 & 0.9090 & 0.5471\\ 
    Normalizer          & 0.5714 & 0.5191 & 0.7603 & 0.4413\\ 
    MaxabsScaler        & 0.7755 & 0.5169 & 0.9008 & 0.5538\\ 
    MinmaxScaler        & 0.7755 & 0.5178 & 0.9256 & 0.5509\\ 
    PowerTransformer    & 0.7755 & 0.6170 & - & 0.5432\\ 
    QuantileTransformer & 0.7959 & 0.5536 & 0.8842 & 0.5480\\ 
    \bottomrule
  \end{tabular}
\end{table}


\jn{Are we able to get the following conclusion from Fig 1?} \Danrui{I add table with different accuracy of same operator on different downstream ML models.} What is more, the same feature preprocessing pipeline gives different performance when the downstream ML models are different, even the datasets are same. This conclusion can be also derived from Table \ref{tab:acc_order_impact_same_dataset}. In Table \ref{tab:acc_order_impact_same_dataset}, although we just apply the same feature preprocessing pipeline with only one preprocessor on the Forex dataset, when the downstream ML models are different, the performances are different. For example, \textit{PowerTransformer} can achieve 61.70\% accuracy when downstream ML model is LR, while there is only 53.55\% when downstream model is MLP.
Thus, even the datasets are same, with different downstream ML model, we still need various feature preprocessing pipelines. It is hard to find a general pipeline which can handle all occasions. 

\begin{table}[t]% h asks to places the floating element [h]ere.
  \caption{The accuracy of applying preprocessors on Forex dataset with different ML models.}
  \label{tab:acc_order_impact_same_dataset}
  \begin{tabular}{p{0.3\linewidth}<{\centering}
                  p{0.17\linewidth}<{\centering}
                  p{0.17\linewidth}<{\centering}
                  p{0.17\linewidth}<{\centering}}
    \toprule
    \textbf{Preprocessor} & \textbf{LR} & \textbf{XGB} & \textbf{MLP}\\ 
    \midrule
    Binarizer           & 0.5173 & 0.5173 & 0.5173\\ 
    Standardizer        & 0.5928 & 0.5740 & 0.5282\\ 
    Normalizer          & 0.5191 & 0.5309 & 0.5365\\ 
    MaxabsScaler        & 0.5169 & 0.5741 & 0.5318\\ 
    MinmaxScaler        & 0.5178 & 0.5743 & 0.5333\\ 
    PowerTransformer    & 0.6170 & 0.5741 & 0.5355\\ 
    QuantileTransformer & 0.5536 & 0.5743 & 0.5359\\ 
    \bottomrule
  \end{tabular}
\end{table}

\fi



\subsection{Problem Formulation} 
We formally define the Auto-FP problem.

\begin{definition}[Feature Preprocessor]
%Given a column $C$, let $c_i$ be its $i$-th element. A preprocessor $\mathcal{P}$ is a mapping function that maps column $C$ to column $C'$, where each $c_i$ is mapped to $c_i'$.
Given a dataset $D$, let $r_i$ be its $i$-th row and $c_j$ be its $j$-th column. A preprocessor $\mathcal{P}$ is a mapping function that maps dataset $D$ to $D'$, where each row $r_i$ is mapped to $r_i'$ and each column $c_j$ is mapped to $c_j'$.
\end{definition}

\begin{example}
This paper considers the seven feature preprocessors from Section~2.1. Given a dataset $D$ and a feature preprocessor $\textit{StandardScaler}(\cdot)$, we have $D' = \textit{StandardScaler}(D)$.
\end{example}

\begin{definition}[Feature Preprocessing Pipeline]
%Given a set of preprocessors, a pipeline $\mathcal{L}$ of size $n$ is a composite function that contains a sequence of $n$ preprocessors, denoted by $\mathcal{P}_1 \rightarrow \mathcal{P}_2 \rightarrow \cdots \rightarrow \mathcal{P}_n$. For a column $C$, $\mathcal{L}$ maps it to column $C'$, where $C' = \mathcal{P}_n \circ (...\mathcal{P}_2 \circ (\mathcal{P}_1(C))$. For a dataset $\mathcal{D}$ where $\mathcal{C}_i$ is $i$-th column, $\mathcal{L}$ maps it to dataset $\mathcal{D}'$, where $\mathcal{C}_i' = \mathcal{P}_n \circ (...\mathcal{P}_2 \circ (\mathcal{P}_1(\mathcal{C}_i))$.
Given a set of preprocessors, a pipeline $\mathcal{L}$ of size $n$ is a composite function that contains a sequence of $n$ preprocessors, denoted by $\mathcal{P}_1 \rightarrow \mathcal{P}_2 \rightarrow \cdots \rightarrow \mathcal{P}_n$. For a dataset $\mathcal{D}$, $\mathcal{L}$ maps it to dataset $\mathcal{D}'$, where $\mathcal{D}' = \mathcal{P}_n \circ (...\mathcal{P}_2 \circ (\mathcal{P}_1(\mathcal{D}))$.
\end{definition}

\begin{example}
Given a dataset $\mathcal{D}$ and a feature preprocessing pipeline
$\textit{PowerTransformer} \rightarrow \textit{MinmaxScaler} \rightarrow \textit{Normalizer}$,
we have
\[
\mathcal{D}' = \textit{Normalizer} \circ \bigl(\textit{MinmaxScaler} \circ (\textit{PowerTransformer}(\mathcal{D}))\bigr).
\]
\end{example}

\stitle{Pipeline Error.} Auto-FP problem is the problem of searching the best pipeline. To solve this problem, we first need to define what the ``\emph{best}'' means, i.e., how to measure the quality of a given pipeline. 

Consider the model training process that gives a classifier $\mathcal{C}$, a training dataset $\mathcal{D}_{train}$ with its labels, and a validation dataset $\mathcal{D}_{valid}$ with its labels. For a pipeline $\mathcal{L}$, it will be used to transform the training data $\mathcal{D}_{train}$ and get a new dataset $\mathcal{L}(\mathcal{D}_{train})$. Then, the classifier $\mathcal{C}$ will be trained on the new dataset. We denote the trained classifier as $\mathcal{C}_{\mathcal{L}(\mathcal{D}_{train})}$, or $\mathcal{C}_{\mathcal{L}}$ for simplicity when the context is clear. Clearly, a good pipeline should be the one that minimizes the error of the trained classifier $\mathcal{C}_{\mathcal{L}}$. Since the test data is not available in the training stage, we measure the validation error of $\mathcal{C}_{\mathcal{L}}$ on $\mathcal{D}_{valid}$, denoted by $\validerror(\mathcal{C}_{\mathcal{L}}, \mathcal{D}_{valid})$. Then, we define the error of a pipeline $\mathcal{L}$ as:
\begin{equation}
    \error(\mathcal{L}) := \validerror(\mathcal{C}_{\mathcal{L}(\mathcal{D}_{train})}, \mathcal{D}_{valid})
\end{equation}

Now we have defined the error of a pipeline. Next, we formally define the pipeline search problem (i.e., automated feature preprocessing) in \cref{def:pipe-search}.

\begin{definition}[Automated Feature Preprocessing]
\label{def:pipe-search}
Given a set of preprocessor $\mathcal{S}_{prep}$, suppose that a feature preprocessing pipeline contains at most $N$ preprocessors. Let $\mathcal{S}_{pipe}$ be the set of all pipelines  constructed with $n = \{1, \cdots, N\}$ preprocessors chosen from $\mathcal{S}_{prep}$. The automated feature preprocessing (Auto-FP) problem aims to find the best pipeline with the minimal error, i.e.,
\begin{equation*}
    \argmin_{\mathcal{L} \in \mathcal{S}_{pipe} } \error(\mathcal{L})
\end{equation*}
\end{definition}

%\jn{What's the relationship between pipeline search and automated feature preprocessing? I thought they are the same problem, but based on the following paragraph, they seem different.} \Danrui{The following paragraph is the previous writting before I wrote the strict definitions. Now I have deleted this part and added two examples for illustration for Definition 1 and 2. Actually you're right, pipeline search and Auto-FP are the same problem.}

%\begin{example}
%If a training data $\mathcal{D}_{train} = (X_{train}, Y_{train})$, a validation data $\mathcal{D}_{valid} = (X_{valid}, Y_{valid})$, a library of 7 feature preprocessors $\mathcal{P}$ and a fixed downstream classifier $\mathcal{C}$ are given, With $\mathcal{P}$, a feature preprocessing pipeline set $\mathcal{L}$ can be constructed including pipelines with different lengths from 1 to 7, such as \textit{StandardScaler(·)} and \textit{PowerTransformer(MinMaxScaler(·))}. The automated feature preprocessing problem is to identify the optimal preprocessing pipeline $\ell^{*} \in \mathcal{L}$ operated on $\mathcal{D}_{train}$, such that the resulting classifier $\mathcal{C}$ can get maximal validation accuracy on $\ell^{*} (\mathcal{D}_{valid})$.
%\end{example}


%\begin{align*}
%    \ell_{\Lambda}^{*} = argmax \ acc(\mathcal{C}_{\ell_{\lambda}}^{*}),\\ where \  \Lambda \subset \Lambda_{1} \times \Lambda_{2} \times \cdots \Lambda_{k}
%\end{align*}
%In other words, if we define loss function $\mathcal{L}$ for resulting model, the feature preprocessing problem can also be defined as 
%\begin{align*}
%    \ell_{\Lambda}^{*} = argmin \ \mathcal{L}(\mathcal{C}_{\ell_{\lambda}}, \mathcal{D}_{train}, \mathcal{D}_{valid}), \\
%    where \  \Lambda \subset \Lambda_{1} \times \Lambda_{2} \times \cdots \Lambda_{k}
%\end{align*}

\subsection{Auto-FP as HPO and NAS}
Interestingly, Auto-FP can be viewed in two different ways: either as HPO or NAS.  %As we mentioned before, Automated Feature Preprocessing problem can be formatted as hyperparameter optimization and neural architecture search problem. Now we explain how to transfer Auto-FP problem into the two well-studied problems. 
%\jn{unfinished?} \Danrui{It is finished. And I think it can form a single subsection.}


\begin{figure}[t]
\vspace{-5em}
% \vspace{-2em}
\centering
\subfigure{
\label{Fig.sub.4}
\includegraphics[width=0.9\linewidth]{figures/cash.pdf}}
\subfigure{
\label{Fig.sub.5}
\includegraphics[width=0.9\linewidth]{figures/autofp_as_cash.pdf}}
\vspace{-1em}
\caption{The analogy between HPO and Auto-FP.}\vspace{-1em}
\label{fig:autofp_as_hpo}
\end{figure}

\stitle{Auto-FP as HPO.} HPO aims to find the best combination of classifier and its related hyperparameters for a given dataset. Since different classifiers have different HP space (e.g., LR needs to tune ``penalty'' while Random Forest (RF) does not), its search process contains two  steps and can be modeled as a search tree like Figure~\ref{fig:autofp_as_hpo}(a).  The first step is to select a classifier to activate its corresponding HP space (e.g., RF). The second step is to determine the candidate option for each HP (e.g.,  n\_estimators = 200).  The search process of Auto-FP can also be divided into two steps as shown in Figure~\ref{fig:autofp_as_hpo}(b). The first step is to select the pipeline length (e.g., len = 7). The second step is to determine the specific preprocessor for each position (e.g., $P_1$ = Normalizer). 


%Hyperparameter Optimization is a very traditional problem aiming to find the best combination of classifier and its related hyperparameter for a given dataset. That is, the combination can perform best accuracy on given dataset. HPO is a iterative process. For each iteration, its search process which includes two main steps can be extracted as a search tree like Figure \ref{fig:autofp_as_hpo} shows. Due to the different HP spaces of different classifiers (LR has the HP "penalty" while RF does not have), the first step of HPO problem is selecting a classifier to activate its corresponding HP space. As Figure \ref{fig:autofp_as_hpo} (a) shows, at the first step, Random Forest classifier is selected, and the corresponding HPs n\_estimators and criterion are activated. At the second step, one combination of activated HPs is selected from their candidate options. In Figure \ref{fig:autofp_as_hpo} (a), one combination of activated HPs, i.e. n\_estimators and criterion can be generated. And the HP n\_estimators has 4 options: 100, 200, 500 and 1000.

%With the same logic of search process for each iteration, Auto-FP can also form a search tree with two main steps as Figure \ref{fig:autofp_as_hpo} shows. Due to the different lengths of pipeline are related to different pipeline spaces, the first step of Auto-FP is selecting the length of pipeline and activating its related pipeline space, which is very similar with selecting classifier in HPO problem. As Figure \ref{fig:autofp_as_hpo} (b) shows, at the first step, the pipeline length 7 is selected and a pipeline space with 7 preprocessor positions is activated. At the second step, one combination of activated positions is selected with candidate preprocessors. In Figure \ref{fig:autofp_as_hpo} (b), one combination of activated positions, i.e. $P_1$ to $P_7$ can be generated. And $P_1$ to $P_7$ all have 7 candidate preprocessors as we mentioned in Section 2.1.

%With the very similar formats of these two problems, search algorithms from HPO area like \textit{TPE} and \textit{SMAC} to solve HPO problem can be directly used to solve Auto-FP problem.

%The previous works Auto-WEKA\cite{Auto-WEKA} and Auto-Sklearn\cite{Auto-Sklearn} focus on \textit{Combined Algorithm Selection and Hyperparameter optimization (CASH)} problem, which aims to jointly find the proper algorithms and its own hyperparameters with minimal validation loss of input data. We try to formalize Auto-FP problem with the similar formualtion of CASH problem, which means they can be solved with the same search algorithms.

%\begin{definition}[CASH Problem]
%Assume there are a set of algorithms $\mathcal{A} = \{A_1, A_2, \cdots, A_{m}\}$ and their corresponding domains of hyperparameters $\Lambda_1, \Lambda_2, \cdots, \Lambda_{m}$. The corresponding hyperparameters means only when $A_1$ is selected, its own domain of hyperparameters $\Lambda_1$ is activated. Given a dataset $D = {D_{train}, D_{valid}}$, the algorithms $A_{i} \in \mathcal{A}$ can be trained on $D_{train}$ and validated on $D_{valid}$ with different hyperparameters $\labmda \in \Lambda_{i}$. The CASH problem is to jointly find the optimal algorithm $A^{*} \in A$ and its corresponding hyperparameter $\lambda^{*} \in \Lambda^{*}$ where the loss can be minimized:
%\begin{equation*}
%    A^{*}, \lambda^{*} = \argmin_{A_{i} \in \mathcal{A}, \lambda \in \Lambda_{i}} loss(A^{\lambda}_{i}, D_{train}, D_{valid})
%\end{equation*}
%\end{definition}

%\begin{definition}[Auto-FP as CASH Problem]
%Given a set of preprocessor $\mathcal{S}_{prep}$, assume the feature preprocessing pipelines include $N$ preprocessors at most, let $\mathcal{S}_{pipe} = \{{\mathcal{S}_{pipe}}_{1}, {\mathcal{S}_{pipe}}_{2}, \cdots, {\mathcal{S}_{pipe}}_{N}\}$ be the set of feature preprocessing pipelines with $1, 2, \cdots, N$ preprocessors. The Auto-FP as CASH Problem is to jointly find the optimal pipeline length $n \in \{1, 2, \cdots, N\}$ and its corresponding pipeline $\mathcal{L} \in {\mathcal{S}_{pipe}}_{N}$ with the minimal error, i.e.
%\begin{equation*}
%    n^{*}, \mathcal{L}^{*} = \argmin_{n \in \{1, \cdots, N\}, \mathcal{L} \in {\mathcal{S}_{pipe}}_{n} } \error(\mathcal{L})
%\end{equation*}
%\end{definition}

\begin{figure}[t]
\vspace{-5em}
% \vspace{-2em}
\centering
\subfigure{
\label{Fig.sub.4}
\includegraphics[width=0.9\linewidth]{figures/nas.pdf}}
\subfigure{
\label{Fig.sub.5}
\includegraphics[width=0.9\linewidth]{figures/autofp_as_nas.pdf}}
\vspace{-1em}
\caption{The anology between NAS and Auto-FP.} %\vspace{-1em}
\label{fig:autofp_as_nas}
\end{figure}

\stitle{Auto-FP as NAS.} NAS aims to find the best neural architecture for a given dataset. Auto-FP can be modeled as the chain-structure NAS problem, whose neural architecture has no skip connection among different layers and no multi-branch in each layer. That is, a chain-structure neural architecture is a sequence of operators (i.e., a pipeline) as shown in Figure~\ref{fig:autofp_as_nas}(a).  Its search process optimizes two factors holistically: (1) the max depth of a chain structure; (2) the operator put in each position. Similarly, for Auto-FP, the goal is also to find the best chain-structure neural architecture. The difference is that it puts a feature preprocessor (e.g., Normalizer) rather than a neural-architecture operator at each position.

%Neural Architecture Search is an area aiming to automatically search CNN or RNN which can show best performance on the public dataset like CIFAR-10 or ImageNet. In our paper, we try to make analogy between a special branch of NAS problem, which is Chain-structure NAS problem (as Figure \ref{fig:autofp_as_nas} shows). It is usually used to search good CNN structures. In Chain-structure NAS problem, there is no skip connection among different layers and there is no multi-branch in each layer. The process of Chain-structure NAS problem also cares about two factors: (1) the max depth of a chain structure (2) the operators should be put in each position. Note that the NAS area always tries to search the two things together. 

%The NAS area discretizes the hyperparameters and considers some most commonly used hyperparameters for the operators as single operators, such as $3 \times 3, 5 \times 5, 7 \times 7$ seperable convolutions. Then the above three steps can be collapsed into two steps: (1) Ensure the max depth of a CNN (2) Ensure what operator should be put in each position. 
%The Automated Feature Preprocessing problem also cares about two factors: (1) the max length of a pipeline (3) the preprocessors should be put in each position. Thus the Auto-FP problem can be transferred as the format of Figure \ref{fig:autofp_as_nas} (b). With the very similar formats of these two problems, search algorithms from NAS area like \textit{PNAS} and \textit{ENAS} can be directly used to solve Auto-FP problem.



==> src/categories.tex <==
\section{Categories of Search Algorithm}
\textcolor{blue}{We identify a variety of representative search algorithms from HPO and NAS areas. Table~\ref{tab:summary} shows a summary of these algorithms. Roughly, these algorithms can be divided into 5 categories including traditional, surrogate-model-based, evolution-based, RL-based and band-based algorithms. We introduce these algorithms in details in the following contents.}

\subsection{Traditional Algorithms}
\textcolor{blue}{
There are two traditional methods: random search and anneal. They are all full training algorithms, which
means their training process uses the whole training dataset and trains enough number of iterations. }

\stitle{Random Search.} \textcolor{blue}{Random search is a very traditonal algorithm for hyperparameter tuning problem.
When solving HPO, it considers the space of hyperparameters as a whole space. For example, if a classifier
has 3 hyperparameters and each of them has 3 choices, the whole space has $3 \times 3 = 9$ points. 
At each iteration of random search, the algorithm randomly picks one point from these 9 points and tries it 
on the following classifier. In the automated feature preprocessing scenario, the search space becomes 
the pipelines with different lengths and orders. At each iteration, random search algorithm randomly selects
a pipeline and valid it with downstreaming classifier.}

\stitle{Anneal.} \textcolor{blue}{Anneal is an improved random search algorithm, which always considers the direction of
increasing predicting score. In the traditional HPO scenario, common random search algorithm randomly 
picks up a pipeline to valid. However, the anneal algorithm changes one hyperparameter once a time and 
compares score of current pipeline with current
best score. If the new score is higher than current best, anneal algorithm picks the new score as the best.
With this methodology, the anneal algorithm always promises the upstreaming direction. For the automated
feature preprocessing scenario, at each time, anneal randomly changes one preprocessor of current pipeline 
and compares scores with current best score. 
%\jn{What does ``change'' mean? Does it include adding/removing a preprocessor? }
}

\subsection{Surrogate-Model-based Algorithms}
\textcolor{blue}{There are two algorithm (\textit{TPE} and \textit{SMAC}) which are based on \textit{Sequential Model-based Optimization (SMBO)}. There are three key elements in \textit{SMBO}: 1) a target model $\mathcal{M}$ requiring hyperparameter tuning to get better accuracy. 2) a surrogate model capturing the dependence between hyperparameters $x$ and the error rate of target model $e_x$, denoted by $p(e_x|x)$. In most cases, the surrogate model is gaussian process. 3) an acquisition function used for generating knowledgeable hyperparameters for evaluation. Knowledgeable hyperparameters means these hyperparameters can either reduce the error rate of target model with high probability or reduce the predictive variance. In common cases, the acquisition function is Expected Improvement (EI). 

The pseudo-code of \textit{SMBO} is shown in Algorithm 1. \textit{SMBO} firstly initialize the target model $\mathcal{M}$, then iterating with following steps: 1) generating candidate hyperarameter(s) according to acquisition function. 2) evaluating the generated hyperpaprameter(s) with training set and validation set and getting new error rate. 3) updating surrogate model with newly observed hyperparameter(s). Both \textit{TPE} and \textit{SMAC} follows this iterative structure. And they are all full training algorithms. }


%\textit{Bayesian Optimization} algorithms can balance exploration and exploitation well. 
\stitle{SMAC}. \textcolor{blue}{Traditional sequential model-based optimization utilize the gaussian process to evaluate $p(e_x|x)$. However, the gaussian optimization does not performs well with categorical hyperparameters. \textit{SMAC} uses random forest to solve the poor performance of discrete hyperparameters and handle high-dimensional input data. Also, SMAC can handle conditional hyperparameters by initiating the inactive hyperparameters as their default values. Because random forest is not often used as probability models, for a specified hyperparameter $x$, the value of $p(e_x|x)$ is calculated by the mean and variance ($\mu_x$ and $\sigma_x$) of predictions of single trees, which is $\mathcal{N}(\mu_x, \sigma_x^2)$. With the formula of $p(e_x|x)$, the expected improvement is recalculted by Equation \ref{eq:smac_ei}, } where $u = \frac{e_x^* - \mu_x}{\sigma_x}$. 
\begin{equation}
\label{eq:smac_ei}
    EI(x) = \sigma_x \times [u \times \Sigma(u) + \phi(u)]
\end{equation}

\textcolor{blue}{Thus the process of SMAC following these steps: 1) Initialization: initializing the first evaluation of SMAC is by using the default values of each hyperparameters. 2) Fitting surrogate model: utilizing the current observations to train surrogate random forest model (10 trees by default) 3) Finding candidates: picking up candidates with local and random search 4) Intensification: competing and replacing the currently observed best hyperparameter with candidates. Note that SMAC uses two strategies to promise its robustness. The first strategy is during the parameter selection process, utilizing local search for the 10 observed hyperparameters with highest EI values and randomly picking 10000 hyperparameters in the search space to promise the balance of exploration and exploition. The second strategy is during the intensification process. If a candidate hyperparameter wants to be an incumbent, it must exceed current incumbent on all the evaluated settings. }

\stitle{TPE}.
\textcolor{blue}{Arguing that surrogate models with parametric estimation (gaussian process and random forest) are inefficient, \textit{TPE} proposes another surrogating strategy, that is, instead of modelling $p(e_x|x)$, \textit{TPE} tries to split $p(e_x|x)$ into $p(x|e_x)$ and $p(e_x)$. Note  that the $p(x|e_x)$ is modelled with two non-parametric densities, as Equation \ref{eq:tpe} shows. $\ell(x)$ is the density estimated by observe hyperparameters whose observations are smaller than the threshold $e_x^*$. $g(x)$ is the density estimated by observe hyperparameters whose observations are larger than the threshold $e_x^*$. The threshold $e_x^*$ is the $\gamma$-quantile of current observations. With the new surrogating strategy, the Expected Improvement is proportion to $(\gamma + \frac{g(x)}{\ell(x)} \times (1 - \gamma))^{-1}$. Thus, TPE maximize the EI value by selecting candidate which can minimize $g(x)/l(x)$.}

TPE considers that all the hyperparameters with conditions can construct a tree-structure, which can omit inactive conditional parameters during searching. Besides, considering $p(e_x|x) = \frac{p(x|e_x) p(e_x)}{p(x)}$, TPE gives an 1-D estimator for every node in the tree structure to estimate $p(x)$. Discrete hyperparameters are estimated by their number of occurances in the set of observations. And continuous hyperparameters are estimated by . Comparing the surrogate model of gaussian process, TPE can reduce the time complexity from cubic to linear. 

\begin{equation}
\label{eq:tpe}
p(x|e_x)=
\begin{cases}
$\ell(x)$ & \text{if $e_x < e_x^*$}\\
$g(x)$ & \text{if $e_x \geq e_x^*$}
\end{cases}
\end{equation}

\stitle{PNAS}.
\textcolor{blue}{PNAS is a short name of Progressive Neural Architecture Search, which is a greedy algorithm for searching best neural network structure within limited number of iterations or time. When used in NAS scenario, it starts from simplest cell structures, which is composed by only one block like single convolution layer. Then it expands the simple structure by adding more possible block structures. A surrogate model is used when expanding, which helps select top-k structures to valid with its score prediction. Initially, the surrogate model is trained by the actual validation scores of the simplest structures. With more and more actual generated validation scores, the surrogate model becomes more and more precise.}

\textcolor{blue}{By transferring the PNAS algorithm into our automated feature preprocessing scenario, we initially start with only one single preprocessor as pipeline, then valid them and train the surrogate model (MLP or LSTM). PNAS progressively adds new preprocessors according to the predicting scores of high-level pipelines. }



\subsection{Evolution-based Algorithms}
\textcolor{blue}{Two evolution-based algorithms are Tournament Evolution and PBT. Tournament Evoluation is a full training 
algorithms borrowed from \textit{Neural Architecture Search} area. PBT is also from \textit{NAS} area with 
partial training machinanism.} 

\stitle{Tournament Evolution}. 
\textcolor{blue}{Tournament evolution is an algorithm proposed for solving neural architecture search problem. It employs simple encoding that each individual neural architecture is a single DNA. During each evolution step, $S$ individuals are randomly chose from the population. The validation scores of these structures are compared and the structure with best score are used for reproduction. The mutation ways includes inserting or removing a convolution layer, altering stride number or learning rate, etc. When injecting the newly mutated structure into population, there are two ways of killing bad structures: killing the oldest structure or killing the structure with lowest validation score.}

\textcolor{blue}{Transferring tournament evolution to automated feature preprocessing scenario is simple. The tournament selection way and the killing way are directly employed. However, the mutation is totally different with NAS scenario. There are four types of mutation: (1) randomly adding a preprocessor (2) randomly removing a preprocessor (3) randomly replacing a preprocessor (4) randomly switching the positions of two preprocessors. With above changes, tournament evoluation can be used for solving automated feature preprocessing problem.}

\stitle{PBT}. 
\textcolor{blue}{Comparing with \textit{SMBO} utilizing the slow sequential optimization and non-robust parallel random/grid research, \textit{PBT} tries to bridge the parallel computation and sequential optimization. \textit{PBT} utilize the information shared between different threads. Combining with the idea of evolutionary process, \textit{PBT} proposes a 4-step process: (1) \texttt{step} function performs one step gradient descent to optimize the weights $\theta$ for neural networks under a particular hyperparameter $h$  (2) \texttt{eval} function is used to evaluate the objective function like accuracy on validation set with current model (3) \texttt{exploit} function broadcasts the current best model to the whole population (4) \texttt{explore} function randomly perturbs the hyperparameters to promise the exploration. The 4-step process starts from some random hyperparameters, which is composed as a population, and iteratively call \texttt{step} and \texttt{eval} function until the model meets some requirements, such as the number of training step and the lowest bar of validation accuracy. At this point, all the trials in this population are paused. \textit{PBT} calls the \texttt{exploit} function to replace the weights and hyperparameters of all other trials with the weights and hyperparameters of current best trial. If the replaced trials are not the best trial, after replacing, \textit{PBT} calls the \texttt{explore} function to perturb the hyperparamters and calls the \texttt{eval} function to generate evaluation results. Then, \textit{PBT} update the whole population with new models and new evaluations. The process iterates until the convergence of objective function.} 

\subsection{RL-based Algorithms}
\textcolor{blue}{In reinforcement learning, there are three key elements: actor, environment and reward. Environment produces an observation (or state) into actor. Actor produces an action according to the observation. A reward function can calculate the reward according to the observation and chosen action. After actor taking an action, environment can receive this action and produce new observation according to the input. The process circulates until achieving end conditions. The recording of all observations and taken actions $\tau = \{s_{1}, a_{1}, r_{1}， s_{2}, a_{2}, r_{2}, \cdots, s_{T}, a_{T}, r_{T}\}$ is called a trajectory (or a episode). $S_{i}, a_{i}, r_{i}$ stands for the $i$\-th observation, action and reward. $T$ is the length of the trajectory. The goal of reinforcement learning is to find an optimal policy $\pi_{\theta}$ which can maximize the expected cumulative reward $\hat{R}_{\theta} = \sum_{j = 1}^{T} r_{i}$, which is calculated by the sum of cumulative reward of many samples of trajectory ($\tau$).}

\stitle{REINFORCE}. 
\textcolor{blue}{REINFORCE is a very traditional Monte Carlo Policy Gradient Algorithm, which belongs to reinforcement learning area. Policy gradient algorithm tries to directly update the parameter $\theta$ of an actor by adding the gradient of $\hat{R}_{\theta}$. Especially, REINFORCE employs the idea of stochastic gradient descent, that is, after sampling just one trajectory, updating the parameter $\theta$ when enumerating each observation and action. The algorithm is shown in Algorithm 4. The detailed gradient calculation in line 6 can be found in \textcolor{red}{Appendix A}.}

\stitle{ENAS}. 
\textcolor{blue}{Comparing with other neural architecture search algorithms, \textit{ENAS} proposes the idea of parameter sharing. Inspired by the parameter transferring strategy in transfer learning area, \textit{ENAS} considers all the neural network architectures as DAGs, and considers the whole search space as a large super-graph. The nodes in this super-graph represents local computation, and the edges represents the edge flow. Then, the parameters can be shared among all the sub-graphs, which represents the child models. With this strategy, when choosing the optimum, the child models do not need to be trained from scratch, which is very time and resource consuming. \textit{ENAS} utilizes a LSTM as the controller to predict the edges that should be activated and the computation operators that should be used. With these two primary elements, an neural network structure can be constructed and put into evaluation. Note that the shared weights can be utilized only if its belonged edge is activated.}

\subsection{Band-based Algorithms}
\textcolor{blue}{Hyperband algorithm and BOHB algorithm are all \textit{Band-based} algorithms, which are all partial training methods. \textit{Band-based} algorithms formulate hyperparameter optimization problem as a pure-exploration non-stotachastic infinite-armed bandit problem. They are all mainly based on \textit{Successive Halving} algorithm. The inputs of \textit{Successive Halving} algorithm are the number of hyperparameter \textit{n} and a limited budget \textit{B}. For example, if the budget \textit{B} is set to 1 hour and the number of hyperparameter \textit{n} is set to 64, after the first iteration of \textit{Successive Halving} running with 10 minutes, we keep the top half of hyperparameters and drop the 32 bottom hyperparameters. Each hyperparameter can get about 9 seconds to train. After the second iteration, the top 16 are kept and the bottom 16 are dropped. Each hyperparameter can get about 18 seconds to train, which is two times of hyperparameters training in the first iteration. When the budget (1 hour) is consumed, the best hyperparameter is left and trained for enough time, which is about 10 minutes. However, \textit{Successive Halving} does not consider the trade-off between the number of configurations and the training time for each hyperparameter. Larger number of hyperparameters will cause short training of each hyperparameter and small number of hyperparameters will cause the limited exploration. }

\stitle{Hyperband}. 
\textcolor{blue}{\textit{Hyperband} algorithm tries to solve this trade-off problem by dynamic calculating the number of hyperparameters according to the budget and dynamic allocation of training resources. It considers \textit{Succesive Halving} as a  subroutine and each running of SH is called a bracket. It has two parts: (1) the outer loop controls the number of sampled hyperparameters $n$ and the initial resource allocation $r$ for each bracket. (2) the inner loop is a standard process of \textit{Successive Halving}. During the initialization process of each bracket, the hyperparameters are sampled randomly. The whole process of \textit{Hyperband} is shown in Algorithm 2. The inputs of \textit{Hyperband} includes the minimal resource $b_{min}$ and the maximum resource $b_{max}$ that can be utilized by a single configuration, and a parameter $\eta$ that controls the hyperparameter discarding proportion during the \textit{Successive Halving} process. According to the three inputs, the total number of brackets can be calculated, which is $\lfloor log_{\eta}\frac{b_{max}}{b_{min}} \rfloor + 1$. Different brackets with different number of required hyperparameters create the balance between aggressive evaluations with smaller budgets and promising evaluations with larger budgets.}  

\stitle{BOHB}. 
\textcolor{blue}{By indicating the shortcoming of pure \textit{Hyperband}, that is, randomly generating sampled hyperparameters wastes the limited budgets. If the hyperparameter generating process can be directed, the \textit{Hyperband} will converge to global optimum faster with high probability. Considering the good performance of Bayesian Optimization on hyperparameter optimization and the simplicity of \textit{TPE}, it is a promising way to combine Bayesian Optimization with \textit{Hyperband}, which is \textit{BOHB}. Fundamentally, \textit{BOHB} only changes \texttt{get\_sampled\_hyperparameters($n$)} of Algorithm 2 from purely randomness into Algorithm 3. With the input of a random fraction $\rho$, the sampling process of \textit{BOHB} can give a mixture of randomly selected hyperparameters and hyperparameters generated by \textit{TPE}, which helps to increase exploration and prevent the local optimal problem. When training the \textit{TPE}, \textit{BOHB} always considers the observations with largest budgets and enough points ($>N_{min}$) at current stage, which promises the effectiveness of the surrogate model. Note that in line 11, the $\ell'(x)$ is generated by multiplying a bandwidth $b_w$ with all bandwidth of $\ell(x)$ to strengthen more exploration surrounding the promising hyperparameters.} 





==> src/experiment.tex <==
\vspace{-.25em}
\section{How do different search methods perform?}
In practice, when users are looking for a feature preprocessing pipeline with good quality, they often constrain search time. Thus in this section we investigate how these search methods perform with specified time limits. At first, we compare these algorithms and rank them. Then, we explore the trade-off between time and accuracy. In this end, we analyze  the performance bottleneck of these algorithms and identify the opportunities to further improve them. 

\subsection{Datasets} 
%\jn{Describe how you select the ten datasets.} \Danrui{Done.} 
We search for a large collection of real-world datasets (in total 46 datasets) from the widely-known AutoML challenge website~\cite{AutoML-Challenge-Website}, an AutoML Benchmark~\cite{AutoML-Benchmark} and Kaggle datasets~\cite{Kaggle-Datasets}. Not all datasets can be improved by Auto-FP. Since the goal of our study is to compare different search algorithms, we remove the \emph{easy} datasets. Specifically, we remove (1) the datasets with very high validation accuracy (>95\%) even with a simple downstream ML model like LR and (2) the datasets which can be easily improved to very high validation accuracy (>95\%) even with randomly searched (200 iterations) pipelines. Finally, ten datasets are selected. As shown in Table~\ref{tab:dataset}, these selected datasets have diverse characteristics in terms of dataset size, the number of rows/columns, and binary/multi classification. These broad considerations promise the generalization of our experiments.

\begin{table*}[t]
 \vspace{-5em}
 \caption{All Collected Datasets with Performance of Simple Auto-FP (\textit{RS} for 200 Iterations).}
 \vspace{-1em}
  \centering
  \footnotesize
  \begin{tabular}{|p{0.1\linewidth}<{\centering}
                  |p{0.05\linewidth}<{\centering}
                  |p{0.05\linewidth}<{\centering}
                  |p{0.05\linewidth}<{\centering}
                  |p{0.1\linewidth}<{\centering}
                  |p{0.1\linewidth}<{\centering}
                  |p{0.1\linewidth}<{\centering}
                  |p{0.1\linewidth}<{\centering}
                  |p{0.1\linewidth}<{\centering}
                  |p{0.1\linewidth}<{\centering}|}
    \hline
    \textbf{Dataset} &  \textbf{\# of rows} & \textbf{\# of cols} & \textbf{\# of classes} & \textbf{\makecell{LR Acc \\ (no prep)}} & \textbf{\makecell{LR Acc \\ (200 iter RS)}} & \textbf{\makecell{XGB Acc \\ (no prep)}} & \textbf{\makecell{XGB Acc \\ (200 iter RS)}} & \textbf{\makecell{MLP Acc \\ (no prep)}} & \textbf{\makecell{MLP Acc \\ (200 iter RS)}}\\
    \hline
    ada & 4146 & 48 & 2 & 0.8336 & 0.8536 & 0.8641 & 0.8641 & - & -\\ \hline
    austrilian & 689 & 14 & 2 & 0.8743 & 0.8888 & 0.8454 & 0.8695 & 0.826 & - \\
    \hline
    blood & 747 & 4 & 2 & 0.7733 & 0.8088 & 0.6888 & 0.8088 & 0.7022 & - \\
    \hline
    BNG\_austrilian & 999999 & 14 & 2 & 0.8574 & 0.861 & 0.8732 & 0.8732 & - & - \\ 
    \hline
    christine & 5417 & 1636 & 2 & 0.6678 & 0.7244 & 0.7257 & 0.7318 & - & - \\ 
    \hline
    Click\_prediction\_small & 39947 & 11 & 2 & 0.8311 & 0.8317 & 0.8317 & 0.8344 & - & -\\ 
    \hline
    covtype & 581011 & 54 & 7 & 0.6226 & 0.7234 & 0.8692 & 0.876 & - & - \\ 
    \hline
    credit\_1 & 29999 & 23 & 2 & 0.7785 & 0.8141 & 0.8148 & 0.8177 & - & - \\ 
    \hline
    EEG & 14979 & 14 & 2 & 0.6288 & 0.6659 & 0.9325 & 0.935 & - & -\\ \hline
    electricity & 45312 & 8 & 2 & 0.7524 & 0.7544 & 0.91 & 0.9101 & - & - \\ 
    \hline
    emotion & 390 & 77 & 2 & 0.9487 & 0.9572 & 0.8974 & 0.9401 & 0.4529 & - \\
    \hline
    fibert & 8237 & 800 & 7 & 0.6674 & 0.667 & 0.6925 & 0.6949 & - & - \\ 
    \hline
    forex & 43824 & 10 & 2 & 0.5308 & 0.6677 & 0.5734 & 0.6893 & 0.5287 & - \\
    \hline
    gesture & 9872 & 32 & 5 & 0.4541 & 0.5175 & 0.6654 & 0.6667 & - & - \\ 
    \hline
    heart & 302 & 13 & 2 & 0.8461 & 0.8901 & 0.8351 & 0.8461 & 0.5714 & - \\
    \hline
    helena & 65195 & 27 & 100 & 0.2327 & 0.3353 & 0.3376 & 0.3376 & - & - \\ 
    \hline
    higgs & 98048 & 28 & 2 & 0.6416 & 0.6453 & 0.7214 & 0.7226 & - & - \\ 
    \hline
    house\_data & 21613 & 18 & 12 & 0.4878 & 0.6414 & 0.7114 & 0.7131 & - & - \\ 
    \hline
    jannis & 83732 & 54 & 4 & 0.6008 & 0.6522 & 0.7142 & 0.7144 & - & - \\ 
    \hline
    jasmine & 2983 & 144 & 2 & 0.7882 & 0.8055 & 0.8067 & 0.8245 & 0.781 & - \\
    \hline
    kc1 & 2108 & 21 & 2 & 0.8467 & 0.8593 & 0.8546 & 0.8562 & - & -\\ 
    \hline
    madeline & 3139 & 259 & 2 & 0.5732 & 0.5966 & 0.8407 & 0.8471 & 0.5116 & - \\
    \hline
    numerai28.6 & 96319 & 21 & 2 & 0.5254 & 0.5273 & 0.5057 & 0.518 & - & - \\ 
    \hline
    pd\_speech\_features & 755 & 753 & 2 & 0.7488 & 0.8546 & 0.8986 & 0.9074 & 0.7312 & - \\
    \hline
    philippine & 5831 & 308 & 2 & 0.6874 & 0.7234 & 0.7451 & 0.7645 & - & - \\ 
    \hline
    phoneme & 5403 & 5 & 2 & 0.731 & 0.7762 & 0.8908 & 0.8945 & - & - \\ 
    \hline
    thyroid-allhyper & 2799 & 26 & 5 & 0.6667 & 0.7202 & 0.6833 & 0.6988 & 0.6857 & - \\
    \hline
    vehicle & 845 & 18 & 4 & 0.6929 & 0.7598 & 0.7795 & 0.7795 & - & - \\ 
    \hline
    volkert & 58039 & 180 & 10 & 0.5449 & 0.5978 & 0.6925 & 0.6934 & - & - \\ 
    \hline
    wine\_quality & 6496 & 11 & 7 & 0.4628 & 0.5356 & 0.6541 & 0.667 & 0.5079 & - \\
    \hline
    analcatdata\_authorship & 840 & 70 & 4 & 1 & 1 & 0.992 & 1 & - & - \\ 
    \hline
    gas-drift & 13909 & 128 & 6 & 0.9451 & 0.9918 & 0.9935 & - & - & - \\ 
    \hline
    har & 10298 & 561 & 6 & 0.9796 & - & 0.9896 & - & - & -  \\ 
    \hline
    hill & 1211 & 100 & 2 & 1 & 1 & 0.6346 & 1 & - & - \\ 
    \hline
    ionosphere & 350 & 34 & 2 & 0.8952 & 0.9238 & 0.9523 & 0.9523 &  - & - \\ 
    \hline
    isolet & 599 & 617 & 2 & 0.9888 & 0.9944 & 0.9777 & 0.9888 & - & - \\ 
    \hline
    mobile\_price & 1999 & 20 & 4 & 0.6216 & 0.9633 & 0.9233 & 0.9133 & - & - \\ 
    \hline
    mozilla4 & 15545 & 5 & 2 & 0.8512 & 0.9384 & 0.9577 & 0.9579 & - & - \\ 
    \hline
    nasa & 4687 & 33 & 2 & 0.8486 & 0.9864 & 0.995 & 0.995 & - & -\\ 
    \hline
    page & 5472 & 10 & 5 & 0.9482 & 0.9707 & 0.9652 & 0.9742 & - & -\\ 
    \hline
    robot & 5455 & 24 & 4 & 0.686 & 0.8686 & 0.9963 & 0.9963 & - & -\\ 
    \hline
    run\_or\_walk & 88587 & 6 & 2 & 0.7155 & 0.8516 & 0.9913 & 0.9913 & - & -\\ 
    \hline
    spambase & 4600 & 57 & 2 & 0.9 & 0.9347 & 0.9442 & 0.9449 & - & - \\ 
    \hline
    sylvine & 5123 & 20 & 2 & 0.8418 & 0.9219 & 0.9486 & 0.9518 & - & - \\ 
    \hline
    wall-robot & 5455 & 24 & 4 & 0.686 & 0.8686 & 0.9963 & 0.9963 & - & -\\ 
    \hline
    wilt & 4838 & 5 & 2 & 0.9641 & 0.9779 & 0.98 & 0.9876 & - & - \\
    \hline
  \end{tabular}
  \label{tab:dataset}\vspace{-1em}
\end{table*}

\begin{table}[t]
%  \vspace{-1em}
 \caption{Dataset used and their characteristics.}
 \vspace{-1em}
  \centering
  \footnotesize
  \begin{tabular}{|p{0.2\linewidth}<{\centering}
                  |p{0.2\linewidth}<{\centering}
                  |p{0.2\linewidth}<{\centering}
                  |p{0.2\linewidth}<{\centering}|}
    \hline
    \textbf{Dataset} &  \textbf{\# of rows} & \textbf{\# of cols} & \textbf{\# of classes}  \\
    \hline
    Australian~\cite{Australian-Dataset} &  552 & 14 & 2 \\
    \hline
    Blood~\cite{Blood-Dataset}&  598 & 4 & 2 \\
    \hline
    Emotion~\cite{Emotion-Dataset} &  312 & 77 & 2 \\
    \hline
    Forex~\cite{Forex-Dataset} &  35060	& 10 & 2 \\
    \hline
    Heart~\cite{Heart-Dataset} &  242 & 13	& 2 \\
    \hline
    Jasmine~\cite{Jasmine-Dataset} &  2387 & 144 & 2 \\
    \hline
    Madeline~\cite{Madeline-Dataset}&  2512 & 259	& 2 \\
    \hline
    Pd~\cite{Pd-Dataset} &  604 & 753 & 2 \\
    \hline
    Wine~\cite{Wine-Dataset} &  5197 & 11 & 7  \\
    \hline
    Thyroid~\cite{Thyroid-Dataset} &  2240	& 26 & 5 \\
    \hline
  \end{tabular}
  \label{tab:dataset}\vspace{-1em}
\end{table}


\subsection{Experimental Setup} \label{exp-setup}


\stitle{Search Algorithms.} As shown in Table \ref{tab:summary}, we consider 15 search algorithms in total. Some of them have been included in famous \texttt{Python} libraries. E.g., \texttt{HyperOpt} \cite{Hyperopt} %\jn{add citation} \Danrui{Added.}
includes \textit{Anneal} \cite{Anneal} and \textit{TPE}, \texttt{SMAC3} \cite{SMAC3} 
%\jn{add citation} \Danrui{Added.} 
includes \textit{SMAC} algorithm, and \texttt{HyperbandSter} \cite{HpBandSter}
%\jn{add citation}\Danrui{Added}%
includes \textit{Hyperband} and \textit{BOHB}. We slightly change these libraries to make their algorithms support our scenario. For NAS algorithms like \textit{PNAS} and \textit{ENAS}, they are originally implemented in \texttt{PyTorch}. However, they do not fit into our scenario, and thus we re-implement them based on their papers. We also implement \textit{REINFORCE}, \textit{Tournament Evolution}, and \textit{PBT}. Note that all algorithms are implemented in \texttt{Python}, which is fair for comparison. 




%there are totally 11 algorithms. Considering the different types of surrogate model (MLP and LSTM) and the ensemble option, PNAS can generate 4 different version of algorithms. Also, considering different killing strategy of Tournament Evolution, the Tournament Evolution can generate two different version of algorithms. Thus, we have 15 algorithms for experiments in total. 


\stitle{Downstream Classifiers.} We evaluate search algorithms using three downstream classifiers: Logistic Regression (LR), XGBoost (XGB) and Multi-layer Perceptron (MLP). Logistic Regression is a linear model, XGBoost is a  tree-based model, and Multi-layer Perceptron is a neural network. They are all very commonly-used, thus our experimental results based on them can provide insights on a wide range of scenarios. In terms of implementation, we use LR (set n\_jobs = 1) and MLP in the Scikit-learn library with default parameters, and use the XGB model (set n\_jobs = 1) in the XGBoost library. 
%The downstream classifiers \jn{replace downstream with downstream for the whole paper.} \Danrui{I have replaced all.} used in our experiments includes \textit{Logistic Regression}, \textit{XGBoost} and \textit{MLP}. There are two reasons that we choose these three models: (1) they are all representative models of their type. \textit{Logistic Regression} belongs to Generalized Linear Model, \textit{XGBoost} is a popular tree-based model composed by many decision trees, and \textit{MLP} is a neural network. (2) they are all popular in practical scenarios. \textit{Logistic Regression} model is broadly used in finance area for detecting fraud or predicting stock price, etc. \textit{XGBoost} is a very popular classifier for many competitions on \texttt{Kaggle}. \textit{MLP} is the most simple neural network which can be expanded to deep neural network. 


\stitle{Training and Evaluation.} 
For each dataset in Table \ref{tab:dataset}, we split it into training and validation. The proportion of training and validation is 80:20. The training set is used to generate trained downstream models after being preprocessed. And the preprocessed validation set is used to evaluate the trained models. Based on evaluations, search algorithms can derive information and choose proper search direction for next steps. After iterative search of preset time limits, search algorithms stop their work and output the feature preprocessing pipeline with highest validation accuracy.
%\jn{remove test set and explain why we use validation accuracy to compare different search algorithms.} \Danrui{Need to check previous paper for the proportion.}
%For each dataset in Table \ref{tab:dataset}, we split it into training and testing. The proportion of training and testing is 80:20, and the validation set takes 20 percent of training set. Thus, the proportion of training, validation, and testing is 64:16:20. The training set is used to generate trained downstream models after being preprocessed. And the preprocessed validation set is used to evaluate the trained models. Based on evaluations, search algorithms can derive information and choose proper search direction for next steps. After iterative search of preset time limits, search algorithms stops their work and output the feature preprocessing pipeline with highest validation accuracy. \jn{remove test set and explain why we use validation accuracy to compare different search algorithms.}
%We repeat each training with five different random seeds (i.e., 0, 42, 167, 578 and 1440) to ensure the reproducibility of our results.

\stitle{Experimental Environment.} We conduct experiments on a guest virtual machine with 110 vCPUs and 970GB main memory.
The guest virtual machine runs on a Linux Kernel-based Virtual Machine (KVM) enabled server equipped with four Intel Xeon E7-4830 v4 CPUs clocked at 2.0GHz and 1TB main memory.
Each CPU has 14 cores (28 hyperthreads) and 35MB Cache.
All of the experiments are repeated five times and we report the average to avoid the influence from hardware and network.



%\subsection{How do these algorithms perform?}
%\subsection{Which algorithm is better?}
%We run the 15 algorithms on the 10 datasets under 6 different time constrains: 60, 300, 600, 1200, 1800 and 3600 seconds. Because of space limitation, we just exhibit the accuracy improvement within 60 seconds in Table \ref{tab:delta_acc_60}. 
%The red text means positive improvement and the green text means the negative improvement. 
%With Table \ref{tab:delta_acc_60}, we can easily get two main insights: \uwave{(1) even with short time limit, these algorithms can enhance the validation accuracy in most cases.} 
%For LR model, these search algorithms give minimum 0.41 percent and maximum 15.75 percent improvement. For XGB model, the improvement is between 0.09 and 9.95 percent. And for MLP model, the improvement is between 0.78 and 44.87 percent. 
%\uwave{(2) the improving levels are different on 3 downstream models.} The LR is a linear model, which is hard to split different classes explicitly when data is becoming more complex. It is sensitive to data changing including linear feature preprocessing. Thus the feature preprocessing can help it a lot.
%to get at lease 1.2 percent improvement. 
%Tree models are not sensitive to the linear preprocessors like \textit{MinMaxScaler}. 
%Thus some non-linear operators like \textit{PowerTransformer} are more effective for improving XGB model. 
%Thus it is much harder to find an effective feature preprocessing pipeline for XGB model comparing with LR model. MLP is also sensitive to data changing like LR. The search algorithms are also easy to get improvement with MLP.

%\subsection{Which algorithm is better?}
%By fixing different time limit, the result schema is shown in Table \ref{tab:schema_max_time}. That is, each dataset with different ML models can be applied different search algorithms with different time limit. Validation accuracy and converge iteration statistics are generated for every single row.
%\begin{table}[htbp]% h asks to places the floating element [h]ere.
%  \caption{Result schema when fixing time limit.}
%  \label{tab:schema_max_time}
%  \footnotesize
%  \begin{tabular}{p{0.1\linewidth}<{\centering}
%                  p{0.11\linewidth}<{\centering}
%                  p{0.13\linewidth}<{\centering}
%                  p{0.11\linewidth}<{\centering}
%                  p{0.1\linewidth}<{\centering}
%                  p{0.2\linewidth}<{\centering}}
%    \toprule
%    Dataset  & ML Model & Max time (s) & Search Alg & Accuracy & Converge Time (s) \\
%  \bottomrule
%\end{tabular}
%\end{table}
%We rank search algorithms in limited time with two factors: (1) validation accuracy (2) converging time. The validation accuracy is more important than converging time.
%To figure out which algorithm is better with limited time, we consider from 2 perspective: 1) average validation accuracy 2) average converging time. The importance of accuracy is prior than average converging time. That is if two search methods achieve the same average validation accuracy, the method with smaller average converging time wins. Also with this ranking strategy, for each dataset with each classifier (i.e. LR, XGB and MLP), if the time limit is fixed, a ranking can be generated. 

%\textbf{\textit{Example 2.}} When classifying the \textit{Forex} dataset with \textit{XGB} classifier, if we fix the max running time as 60s, the performance of different search algorithms are shown in Table \ref{tab:example2}. For generating ranking of these algorithms, firstly ranking the Accuracy column to get algorithm ranking according to validation accuracy. In this example, \textit{PBT} is the rank 1 algorithm because it has the best validation accuracy. \text{Anneal} is the rank 2 algorithm. When comparing search algorithms with same validation accuracy like \textit{PNAS\_MLP\_NO\_ENSEMBLE} and \textit{PNAS\_MLP\_ENSEMBLE}, the converging time of these two algorithms are compared. Actually, the converging time of \textit{PNAS\_MLP\_NO\_ENSEMBLE} is smaller than \textit{PNAS\_MLP\_ENSEMBLE}. Thus, \textit{PNAS\_MLP\_ENSEMBLE} is the better algorithm, as Table \ref{tab:example2} shows.

%\begin{table}[htbp]% h asks to places the floating element [h]ere.
%  \caption{Performance of different search algorithms on Forex dataset with XGB model and 60s time limit.}
%  \label{tab:example2}
%  \footnotesize
%  \begin{tabular}{p{0.1\linewidth}<{\centering}
%                  p{0.11\linewidth}<{\centering}
%                  p{0.13\linewidth}<{\centering}
%                  p{0.15\linewidth}<{\centering}
%                  p{0.1\linewidth}<{\centering}
%                  p{0.17\linewidth}<{\centering}}
%    \toprule
%    \textbf{Dataset} & \textbf{ML Model} & \textbf{Max time (s)} & \textbf{Search Alg} & \textbf{Accuracy} & \textbf{Converge Time (s)} \\
%    \midrule
%    Forex & XGB & 60 & RS & 0.6312 & 21.24\\
%    Forex & XGB & 60 & Anneal & 0.6318 & 38.54\\
%    Forex & XGB & 60 & TPE & 0.6093 & 31.31\\
%    Forex & XGB & 60 & SMAC & 0.6106 & 56.04\\
%    Forex & XGB & 60 & TEVO\_H & 0.6219 & 27.45\\
%    Forex & XGB & 60 & TEVO\_Y & 0.6219 & 27.43\\
%    Forex & XGB & 60 & REINFORCE & 0.5278 & 38.46\\
%    Forex & XGB & 60 & ENAS & 0.5301 & 30.95\\
%    \textbf{\textcolor{blue}{Forex}} & \textbf{\textcolor{blue}{XGB}} & \textbf{\textcolor{blue}{60}} & \textbf{\textcolor{blue}{PMNE}} & \textbf{\textcolor{blue}{0.5743}} & \textbf{\textcolor{blue}{32.22}}\\
%    \textbf{\textcolor{blue}{Forex}} & \textbf{\textcolor{blue}{XGB}} & \textbf{\textcolor{blue}{60}} & \textbf{\textcolor{blue}{PME}} & \textbf{\textcolor{blue}{0.5743}} & \textbf{\textcolor{blue}{33.64}}\\
%    Forex & XGB & 60 & PLNE & 0.5961 & 31.40\\
%    Forex & XGB & 60 & PLE & 0.5743 & 24.58\\
%    Forex & XGB & 60 & HYPERBAND & - & -\\
%    Forex & XGB & 60 & BOHB & - & -\\
%    \textbf{\textcolor{red}{Forex}} & \textbf{\textcolor{red}{XGB}} & \textbf{\textcolor{red}{60}} & \textbf{\textcolor{red}{PBT}} & \textbf{\textcolor{red}{0.6666}} & \textbf{\textcolor{red}{26.59}}\\
%  \bottomrule
%\end{tabular}
%\end{table}
%We rank search algorithms in limited time with two factors: \uline{(1) validation accuracy (2) converging time}. The validation accuracy is more important than converging time. Due to many factors impacting search algorithms, such as the time limit and the downstream ML models, we vary granularity for exhibiting ranking results (like Figure~\ref{fig:ranking}). Firstly, we calculate the general ranking for each algorithm. The general ranking means that the ranking aggregates over all datasets, ML models and time limits. Then we group by ML models and time limits to observe if there is any difference comparing with what we observed in general ranking. 
%Rankings of search algorithms with different granularities are shown in Table \ref{tab:general_rank_max_time}, \ref{tab:rank_time_max_time} and \ref{tab:rank_model_max_time}. 

%\begin{figure}[h]
%\centering
%\includegraphics[width=\columnwidth]{figures/ranking.pdf}
%\caption{Ranking of search algorithms. (a) General ranking (b) Ranking with different time limits (c) Ranking with different downstream ML models}
%\label{fig:ranking}
%\end{figure}
%The impact of search algorithms depends on many factors, such as the search time constrains and the downstream ML models. Thus, varying granularity for analysing experiment results is important. Firstly, we calculate the general average ranking for each algorithm. The general ranking means that it aggregates over all datasets, ML models and time limits. Then we group by ML models and time limits to observe if there is any difference comparing with what we observed in general ranking. Rankings of search algorithms with different granularities are shown in Table \ref{tab:general_rank_max_time}, \ref{tab:rank_time_max_time} and \ref{tab:rank_model_max_time}  . 

%\begin{table}[htbp]% h asks to places the floating element [h]ere.
%  \caption{General ranking of different search algorithms.}
%  \label{tab:general_rank_max_time}
  %\large
  %\footnotesize
  %\resizebox{linewidth}{10mm}{
%  \begin{tabular}{p{0.45\linewidth}<{\centering} p{0.45\linewidth}<{\centering}}
%    \toprule
%    \textbf{Search Alg} & \textbf{General Ranking}  \\
%    \midrule
%    RS & 4\\
%    Anneal & 12\\
%    \midrule
%    TPE & 7\\
%    SMAC & 8\\
%    \midrule
%    TEVO\_H & 3\\
%    TEVO\_Y & 2\\ 
%    PBT & 1\\
%    \midrule
%    REINFORCE & 10\\
%    ENAS & 15\\
%    \midrule
%    HYPERBAND & 11\\
%    BOHB & 14\\
%    \midrule
%    PMNE & 5\\
%    PME & 6\\
%    PLNE & 9\\
%    PLE & 13\\
%  \bottomrule
%\end{tabular}
%\end{table}

%\begin{table}[htbp]% h asks to places the floating element [h]ere.
%  \caption{Ranking of different search algorithms under different time limits.}
%  \label{tab:rank_time_max_time}
  %\footnotesize
%  \begin{tabular}{p{0.18\linewidth}<{\centering} 
%                  p{0.085\linewidth}<{\centering}
%                  p{0.085\linewidth}<{\centering}
%                  p{0.085\linewidth}<{\centering}
%                  p{0.085\linewidth}<{\centering}
%                  p{0.085\linewidth}<{\centering}
%                  p{0.085\linewidth}<{\centering}}
%    \toprule
%    \textbf{Search Alg} & \textbf{60} & \textbf{300} & \textbf{600} & \textbf{1200} & \textbf{1800} & \textbf{3600} \\
%    \midrule
%    RS     & 4 & 4 & 4 & 5 & 6 & 3 \\
%    Anneal & 10 & 11 & 12 & 12 & 14 & 14\\
%    \midrule
%    TPE  & 8 & 6 & 7 & 7 & 8 & 10 \\
%    SMAC & 7 & 8 & 10 & 10 & 9 & 9\\
%    \midrule
%    TEVO\_H & 3 & 3 & 3 & 3 & 3 & 5\\
%    TEVO\_Y & 2 & 2 & 1 & 2 & 2 & 4\\ 
%    PBT     & 1 & 1 & 2 & 1 & 1 & 1\\
%    \midrule
%    REINFORCE & 11 & 10 & 8 & 8 & 7 & 8\\
%    ENAS      & 14 & 15 & 15 & 15 & 15 & 15\\
%    \midrule
%    HYPERBAND & 13 & 12 & 11 & 11 & 11 & 11\\
%    BOHB      & 15 & 14 & 13 & 12 & 13 & 13 \\
%    \midrule
%    PMNE & 5  & 5  & 5  & 5  & 4  & 2\\
%    PME  & 6  & 7  & 6  & 4  & 5  & 6\\
%    PLNE & 9  & 9  & 9  & 9  & 10  & 7\\
%    PLE  & 12 & 13 & 14 & 14 & 12 & 12\\
   
%  \bottomrule
%\end{tabular}
%\end{table}

%\begin{table}[htbp]% h asks to places the floating element [h]ere.
%  \caption{Ranking of different search algorithms with different downstream models.}
%  \label{tab:rank_model_max_time}
  %\footnotesize
%  \begin{tabular}{p{0.21\linewidth}<{\centering}
%                  p{0.21\linewidth}<{\centering}
%                  p{0.21\linewidth}<{\centering}
%                  p{0.21\linewidth}<{\centering}}
%    \toprule
%    \textbf{Search Alg} & \textbf{LR} & \textbf{XGB} & \textbf{MLP}  \\
%    \midrule
%    RS & 5 & 4 & 4\\
%    Anneal & 12 & 13 & 12 \\
%    \midrule
%    TPE & 7 & 7 & 8\\
%    SMAC & 9 & 9 & 9\\
%    \midrule
%    TEVO\_H & 3 & 3 & 3\\
%    TEVO\_Y & 2 & 2 & 2\\ 
%    PBT & 1 & 1 & 1\\
%    \midrule
%    REINFORCE & 8 & 11 & 10\\
%    ENAS & 14 & 15 & 15\\
%    \midrule
%    HYPERBAND & 11 & 10 & 13\\
%    BOHB & 13 & 14 & 14\\
%    \midrule
%    PMNE & 4 & 5 & 5\\
%    PME & 6 & 6 & 6\\
%    PLNE & 10 & 8 & 7\\
%    PLE & 15 & 12 & 11\\
%  \bottomrule
%\end{tabular}
%\end{table}

%\textbf{Which search algorithms are the best?} \jn{Do we need to revise this section since Table 3 is updated?} \Danrui{Revised.} \uwave{According to Figure~\ref{fig:ranking}, \textit{TEVO\_H}, \textit{TEVO\_Y} and \textit{PBT} win the top positions in general cases}. Note that they all follow the evolution framework, i.e., \textit{Evolution}-based. No matter how the time limit or the downstream ML model changes, the rankings of the three algorithms are very stable. Thus, when users try to apply Auto-FP on an unfamiliar dataset or downstream model, we recommend users to try \textit{TEVO\_H, TEVO\_Y} or \textit{PBT}. Comparing with other algorithms, the three \textit{Evolution}-based algorithms has the picking-up overhead that is approaching to random search. Also, the three algorithms can promise both exploration and exploition. \textit{TEVO\_H} and \textit{TEVO\_Y} utilize mutation and crossover to promise the exploition, and the random strategy of mutation and crossover promises the exploration. \textit{PBT} uses broadcast to promise exploition and random mutation to promise exploration. Small picking-up overhead and the consideration of both exploration and exploition makes the \textit{TEVO\_H, TEVO\_Y} and \textit{PBT} take top places.


%\textbf{Why surrogate-model-based algorithms are not top algorithms?} Two main reasons causes the worse performance of surrogate-model-based algorithms: \uwave{(1) the lack of training data at the starting stage causes imperfect search direction.} For example, the starting points of \textit{PNAS} are just the 7 pipelines with only one preprocessor. \jn{This is just the initial stage. As the time goes, there will be more pipelines collected.} 
%And \textit{ENAS} has no starting point. The first predicted pipeline generated by \textit{ENAS} is by a randomly parametered LSTM.  
%\uwave{(2)the time-consuming fitting process of surrogate models causes the less evaluation number of pipelines.} For example, \textit{SMAC} needs to train a random forestm, \textit{TPE} needs to fit many KDEs, \textit{PNAS} needs to fit a MLP or LSTM, \textit{BOHB} also employs a KDE, and \textit{ENAS} also includes a LSTM. These surrogate models take longer time to train. Thus within the same time limit, less time is used to evaluate candidate pipelines, which means the not enough training data of updating surrogate models. It is a vicious cycle. Note that algorithms with complex and slow surrogate models like Random Forest and LSTM performs worse. Algorithms with simpler and faster surrogate models like KDE and MLP performs better. The reasons are \uwave{(1) more complex surrogate models need more data to train precisely.} LSTM and Random Forest all need enough data to train a good predicting model. \uwave{(2) the training speed of more complex models is slower.} The training speed of neural network and ensemble models is slow in common cases, which also leads to the lack of evaluated pipelines (training data) during a fixed time limit. 
%For larger datasets with more complex downstream ML models, the picking-up overhead is no longer the bottleneck, which means that the number of evaluated pipelines of each search algorithm is almost equal. Under this scenario, the algorithms based on surrogate models still perform bad, which indicates the most important reason of poor performance is the imprecise surrogate models. 
%For instance, the ranking of \textit{PNAS\_MLP\_NO\_ENSEMBLE} is increasing by time, which is because MLP is a simple enough surrogate model whose training speed is very fast. The fast training speed leaves space for more evaluations of pipelines. With more and more number of evaluations and longer and longer search time, the MLP prediction is more and more precise.
%Although surrogate models can also provide more promising search direction theoretically, the search algorithms \jn{replace searching with search for the whole paper} \Danrui{Replaced.} with surrogate models cannot really produce better results in practice. 
%The main reason is the lack of training data for training surrogate model at the starting stage, which causes imperfect surrogate models producing imperfect search directions. For example, the default number of starting random-searched pipelines in \textit{SMAC} is just 20. Further more, the starting points of \textit{PNAS} are just the 7 pipelines with only one preprocessor. \jn{This is just the initial stage. As the time goes, there will be more pipelines collected.} And \textit{ENAS} has no starting point. The first predicted pipeline generated by \textit{ENAS} is by a randomly parametered LSTM. 

%For smaller datasets with simpler downstream ML models which make the picking-up overhead be the bottleneck of the whole process, the time-consuming fitting process of surrogate models is another reason causing the less evaluation number of pipelines. For example, \textit{SMAC} needs to train a random forest on each search step, \textit{TPE} need to fit many KDEs to generate new candidate pipelines and \textit{PNAS} needs to fit a MLP or LSTM to predict the selection of next step. On the same way, \textit{BOHB} also employs a KDE as \textit{TPE} does, which actually gets less number of evaluated pipelines in our scenario. \textit{ENAS} also includes a LSTM for prediction of next search step, which is also time consuming actually. Comparing these search methods on the type of surrogate models, algorithms with complex and slow surrogate models like \textit{PNAS\_LSTM\_NO\_ENSEMBLE}, \textit{PNAS\_LSTM\_ENSEMBLE}, \textit{SMAC} and \textit{ENAS} performs bad. Algorithms with simpler and faster surrogate models like KDE including \textit{TPE}, \textit{PNAS\_MLP\_NO\_ENSEMBLE}, \textit{PNAS\_MLP\_ENSEMBLE} get better rankings. The reasons are (1) more complex surrogate models need more data to train precisely. LSTM and random forest are all good models in machine learning area. However, they need enough data to train a good predicting model. (2) the training speed of more complex models is slower. The training speed of neural network and ensemble models is slow in common cases, which also leads to the lack of evaluated pipelines (training data) during a fixed time limit. For larger datasets with more complex downstream ML models, the picking-up overhead is no longer the bottleneck, which means that the number of evaluated pipelines of each search algorithm is almost equal. Under this scenario, the algorithms based on surrogate models still perform bad, which indicates the most important reason of poor performance is the imprecise surrogate models. 

%Note that the ranking of \textit{PNAS\_MLP\_NO\_ENSEMBLE} is increasing by time, which is because MLP is a simple enough surrogate model whose training speed is very fast. The fast training speed leaves space for more evaluations of pipelines. With more and more number of evaluations and longer and longer search time, the MLP becomes more and more precise to take leading position of 

%\textbf{Why reinforcement learning-based algorithms perform bad?} There is an important factor named actor in the reinforcement learning-based algorithms like \textit{REINFORCE}. Actually, the actor is like another format of surrogate model, which predicts next step according to current environment. However, the gradient descent promises good exploition and poor exploration, the actor is easily caught into local optimal. 

%\textbf{Why do \textit{Hyperband} and \textit{BOHB} not perform well?} No matter how time limit and downstream ML model change, \textit{Hyperband} and \textit{BOHB} do not perform well. However, in \cite{Hyperband} and \cite{BOHB}, they can perform well on training deep neural networks. \uwave{The reason is that early-stopping strategy does not work well for LR, XGB and MLP}. For DNNs like LeNet, the resource is epoch. The loss curve depicting the correspondence between epoch and loss does not fluctuate very drastically. Thus the training of DNNs benefits more from the early-stopping strategy. 
%In our scenario, the validation accuracy curves fluctuate drastically according to the number of training iterations or estimators. At the starting stage with 3-5 estimators or iterations, the ranking of pipelines is not similar with the ranking under 100 estimators or iterations. However, at the early stage, about 1/3 pipelines including strong ones are stopped. Thus we cannot benefit much from early-stopping because early-stopping can stop powerful pipelines wrongly in the early stage.
%Thus we can conclude that \textit{Band}-based problems do not fit for feature preprocessing pipeline search scenario well. However, in \textcolor{red}{previous paper}, \textit{Band}-based algorithms can perform well on tasks like training deep neural networks. The reason is that for DNNs like LeNet, the resource of \textit{Band}-based algorithms is epoch. The loss curve of DNNs increases more slowly and stable according to the number of epochs, which means their curve does not fluctuate very drastically. Thus the training of DNNs benefits more from the early stopping strategy of \textit{Band}-based algorithms than feature preprocessing pipeline search scenario. 

%In our scenario, the downstream models are not as complex as DNNs, which means actually their validation accuracy curves fluctuate drastically according to the number of training iterations or estimators. At the starting stage with 3-5 estimators or iterations, the ranking of pipelines is not similar with the ranking under 100 estimators or iterations. However, at the early stage, about 1/3 pipelines are stopped which include some strong pipelines. Thus we cannot benefit much from early-stopping because early-stopping can stop powerful pipelines wrongly in the early stage.
%\begin{figure*}[htbp]
%\centering
%\subfigure[LR]{
%\label{Fig.sub.4}
%\includegraphics[width=0.3\textwidth]{figures/lr_curve.eps}}
%\subfigure[XGB]{
%\label{Fig.sub.5}
%\includegraphics[width=0.3\textwidth]{figures/xgb_curve.eps}}
%\subfigure[MLP]{
%\label{Fig.sub.8}
%\includegraphics[width=0.3\textwidth]{figures/mlp_curve.eps}}
%\caption{Validation accuracy of different ML models with the increase of \# of iterations or estimators.}
%\label{fig:partial_training_curve}
%\end{figure*}
%\textbf{Discussion.} In general, there are two main factors impact the search result: (1) the number of evaluations (2) the consideration of both exploition and exploration. The former is more important than the latter. If the number of evaluations are small, like algorithms with complex surrogate models, even spending more time to consider exploition and exploration, the search results are still not good. If the number of evaluations are enough and without considering exploition and exploration, the performance still cannot be the best, like \textit{RS}. Note that \textit{RS} is still a strong baseline. Combining the two factors is the right direction to search for "good" feature preprocessing pipelines. %\jn{This  looks more like a discussion rather than an exp result.} 

%\subsection{Is longer time limit useful?}
%We investigate the trend of top algorithms under different time constrains from 60 seconds to 3600 seconds, which are the improvement trends of \textit{RS}, \textit{TEVO\_H}, \textit{TEVO\_Y} and \textit{PBT} are shown in our Figure~\ref{fig:max_scores_by_time}. The reason of selecting top algorithms is the meaningless of allocating lots of time to algorithms with bad performance. In this subsection, we care about the converge time of algorithms and the representativeness of short time searching. 
%It is obvious that with the increment of search time, the result validation accuracy of each search algorithms is increasing. That is natural because the increment of time means the increase of evaluated preprocessing pipelines, which at least do not decrease the current maximum validation accuracy. In most figures, when the time limit is smaller than 600 seconds (10 minutes), there are obvious improving trends with the increasing of time limit. However, after 600 seconds, the improving speed becomes slower and slower. For investigating whether it is valuable to continue searching after 600 seconds, we calculates the gap between the accuracy of best algorithm with 3600 seconds time constrain and other time limits. 

%\textbf{When do most algorithms converge?}
%From Figure~\ref{fig:max_scores_by_time}, it is obvious that with the increment of search time, the result validation accuracy of each search algorithms is increasing. That is natural because the increment of time means the increase of evaluated preprocessing pipelines, which at least do not decrease the current maximum validation accuracy. In most cases, after 30 minutes, all the algorithms are approaching convergence. Even Figure~\ref{fig:max_scores_by_time} (b)(c) shows improvement after 30 minutes, the accuracy gap between 60 minutes and 30 minutes 

%\textbf{Is short time searching representative?}



%Table \ref{tab:delta_acc_3600_with_others} shows the accuracy gap between best algorithm with 3600 seconds time constrain and other time constrains. By comparing the maximum validation accuracy of these algorithms in 60 seconds with 3600 seconds, we can find that the maximum gap between these two values is 4.07\%, which means the increasing of search time constrain is useful for enhancing the validation accuracy. However, in most cases, the gaps between 3600 seconds and 60 seconds time constrain are smaller than 2\%, which is consistent with the improvement shown in Figure~\ref{fig:max_scores_by_time}.  If users have 600 seconds budget, the gaps become smaller, which means that for most dataset the gaps are about 1\%. The small gaps in short time limits give users who have very limited time a choice of trying these algorithms with just 60 seconds or 600 seconds and selecting the best one. However, if users have more time to run these top algorithms, we still encourage users to search for longer time because longer time search means more evaluated pipeline then means better validation accuracy.

%\jn{I am a bit confused about the definition of $|\Delta \ Acc|$}



%\subsection{What is the bottleneck of running time?}
%In general, all of search algorithms in this paper follows the same strategy: (1) picking-up feature preprocessing pipelines which need to be evaluated (2) preprocessing training and validation dataset with picked pipelines (3) training and validating ML models with preprocessed training and validation dataset. In this section, we want to figure out the bottleneck of the whole process: the picking-up time, the preprocessing time or the evaluating time. We record the time of each part with 10 minutes time limit and draw these time values in Figure~\ref{fig:overhead}. Note that the bar of \textit{Hyperband} and \textit{BOHB} are not shown in Figure~\ref{fig:overhead}, because the two methods mix the pipeline picking-up and evaluation. Moreover, they have partial training part when evaluating, which makes it impossible to record each part separately as other algorithms. 

%\textbf{When the three time parts become bottlenecks?} \emph{Scenario 1}. small dataset, search algorithm with complex surrogate model, and simple downstream ML model. \emph{Scenario 2}. 

%\textbf{How to resolve bottlenecks?} 

%\textbf{Time distribution of different search algorithms.} Different search algorithms have different time distribution, which is shown in Figure~\ref{fig:overhead_aus_made_lr_mlp}. Overall, the non-surrogate-model-based algorithms have very low proportion of picking-up time. The proportion of preprocessing time and evaluating time depends on the datasets and downstream ML models. As for algorithms with surrogate models, longer training of surrogate models are taken, i.e. longer picking-up time. However, whether picking-up time takes large proportion also depends on datasets and downstream ML models.

%\textbf{When does picking-up time become bottleneck?} If the picking-up time becomes bottleneck during search, it should meet requirements from three perspectives: \uwave{(1) Dataset: the input dataset should be small enough, which does not have large number of rows and columns. (2) Search algorithm: the search algorithm should be with complex surrogate model, like RF and LSTM. (3) Downstream ML model: None.} The requirement of the first factor is because only on small datasets, the picking-up time has the opportunity of becoming bottleneck. Otherwise, the preprocessing time or evaluating time will become bottleneck. The requirement of the second factor is because only algorithms with complex surrogate models spend lots of time for training surrogate models, which is included in picking-up time. Figure~\ref{fig:overhead_aus_made_lr_mlp} illustrates the three requirements. As Figure~\ref{fig:overhead_aus_made_lr_mlp} (a) (b) shows, even with \textit{Australian} dataset, the picking-up time of algorithms without surrogate model or without complex surrogate model cannot be the bottleneck. The picking-up time of algorithms with complex surrogate model like \textit{SMAC} and \textit{PNAS\_LSTM\_NO\_ENSEMBLE} becomes bottleneck, no matter the downstream ML model is LR or MLP. However, when dataset becomes larger, like \textit{Madeline}, the picking-up time of algorithms with complex surrogate model (except \textit{PNAS\_LSTM\_ENSEMBLE}, because its surrogate model is too complex) is not the bottleneck, as Figure~\ref{fig:overhead_aus_made_lr_mlp} (c) (d) shows. Considering scalability of Auto-FP, reducing the picking-up time of search algorithms only contributes limited scenarios like small datasets. It is more meaningful to focus on optimizing preprocessing time on larger dataset and reducing training time of classifier like MLP.


%\textbf{When does preprocessing time become bottleneck?} If the preprocessing time becomes bottleneck, it should be in the two scenarios. The first scenario meets following requirements: \uwave{(1) Dataset: the input dataset should be with small size (2) Search algorithm: without surrogate model (3) Downstream ML model: simple model like LR.} The second scenario meet following requirements: \uwave{(1) Dataset: the input dataset should be with large size (2) Search algorithm: None. (3) Downstream ML model: simple model like LR.} In the first scenario, picking-up time of search algorithms without surrogate model is short, and evaluating time is also small with small dataset and simple downstream model, the side effect of which is the increase of number of evaluations, i.e. preprocessing time becomes bottleneck. Some bars in Figure~\ref{fig:overhead_aus_made_lr_mlp} (a) belongs to the first scenario. In the second scenario, even the dataset is large, the simple downstream model causes short evaluating time. Due to the large dataset, the preprocessing time cannot be neglected and the opportunity of becoming bottleneck is high when downstream model is simple. Figure~\ref{fig:overhead_aus_made_lr_mlp} (c) belongs to the second scenario. 


%\textbf{When does evaluating time become bottleneck?} If the picking-up time becomes bottleneck during search, it also should meet requirements from three perspectives: \uwave{(1) Dataset: the input dataset should be with large size. (2) Search algorithm: None. (3) Downstream ML model: the downstream ML model should be complex, like XGB and MLP.} Complex downstream ML model with large dataset requires lots of training time with the side-effect of reducing the number of evaluations, i.e. picking-up time and preprocessing time. Thus the evaluating time has the opportunity to become the bottleneck. From Figure~\ref{fig:overhead_aus_made_lr_mlp}, we know that (1) even with \textit{Australian} dataset, when the downstream ML model becomes MLP, most search bottleneck becomes evaluating time. (2) even with \textit{Madeline} dataset, when the downstream ML model is as simple as LR, most search bottleneck becomes preprocessing time. (3) when combining \textit{Madeline} and MLP, the evaluating time definitely becomes bottleneck. The requirements can also be generalized into other datasets and downstream ML model like XGB. As Figure~\ref{fig:overhead_forex_made_xgb} shows, the \textit{Forex} dataset has large number of rows which is over 40k. When the downstream ML model is XGB, the bottleneck is evaluating time. So does \textit{Madeline} with XGB.

%From model perspective, in general case, the evaluation time of Logistic Regression is not the bottleneck in binary classification scenario. However, if the dataset is multi-classification (Wine\_quality) dataset, the evaluation time becomes bottleneck because multi-classification is more complex than binary classification problem. Note that the time of preprocessing part also cannot be neglected. For small dataset like Australian with random search algorithm, the smaller picking-up overhead leads to more evaluations. With the small evaluation time of LR on small dataset, the preprocessing part becomes the bottleneck. 
%Whether the training time of downstream XGBoost is bottleneck depends on the datasets and search algorithms. For small dataset Australian, Blood, Emotion and Heart, the picking time of \textit{TPE}, \textit{SMAC}, \textit{PNAS\_LSTM\_NO\_ENSEMBLE} and \textit{PNAS\_LSTM\_ENSEMBLE} is the bottleneck of whole process. For other larger datasets, the bottleneck becomes the evaluation time of XGBoost. For the multi-classification datasets Wine\_quality and Thyroid\_allhyper, the evaluation time is also the bottleneck because it takes much more time to train a XGBoost on multi-classification problems.  
%When downstream model is MLP, the evaluation time becomes the bottleneck in most cases because the complexity of evaluating MLP comparing with LR and XGB. However, there are also some exceptions. For smaller datasets like Australian, Blood, Emotion and Heart, the picking up time of search algorithms with complex surrogate models still becomes the bottleneck because the evaluation time of MLP on small datasets are short.

%From dataset perspective, the size of datasets impacts the proportion preprocessing time a lot. the preprocessing time of small dataset like Australian is also small, thus the bottleneck mainly depends on the picking time of search algorithms and the evaluation time of downstream ML models. If the evaluation time is larger, then it becomes the bottleneck. Otherwise the picking-up overhead of search algorithms becomes the bottleneck. The dataset like Forex has larger number of rows without too high dimension comparing with Australian dataset, thus it has reasonable larger preprocessing time. The bottleneck also depends on search algorithms and downstream ML models. Jasmine, Madeline and Pd\_speech\_features dataset have significant preprocessing time because of their high dimension, even though the downstream ML model is MLP. Thus with simple downstream LR model, preprocessing time is the obvious bottleneck. With more complex downstream XGB and MLP model, the bottleneck becomes their evaluation time because more complex models also takes longer time for training high-dimensional datasets. Multi-classification datasets like Wine\_quality are complex. They lead to the longer training time for all downstream classifiers, even though the size of dataset is not so large. Thus in general, the bottleneck of multi-classification datasets is the evaluation time of downstream model.

%From search method perspective, the search methods based on complex surrogate models including \textit{TPE}, \textit{SMAC}, \textit{ENAS}, \textit{PNAS\_LSTM\_NO\_ENSEMBLE} and \textit{PNAS\_LSTM\_ENSEMBLE} need longer time for picking-up a new pipeline. Algorithms with shorter picking-up time show the bottleneck of preprocessing (simple ML model like LR) or evaluation (complex ML model like XGB and MLP). The picking-up overhead of \textit{Evolution}-based algorithms are very similar. 

%In conclusion, there are three factors can be a bottleneck of search: (1) picking-up time (2) preprocessing time (3) evaluatin time. Which part is the bottleneck depends on search algorithm, datasets and doenstreaming ML models. Knowing where the bottleneck is from, in practice, if users need to speed up the running time, sampling and column selecting are two practical ways to reduce evluation time and preprocessing time from dataset perspective. Also, from search algorithms perspective, users should avoid choosing method with large picking-up overhead like \textit{PNAS\_LSTM\_NO\_ENSEMBLE} and textit{PNAS\_LSTM\_ENSEMBLE}. 

%\section{Outline of Section 4}
%As Section 4 Mentioned.
\subsection{How Do Search Algorithms Perform?}
We run the 15 algorithms on 10 datasets under 6 different time constrains: 60, 300, 600, 1200, 1800 and 3600 seconds. Due to the space constraint, we select the results on some representative datasets and time constraints to report and put other results in our technical report~\cite{Auto-FP}.
%\jn{change the citation to a paper rather than a url}
%\jn{Add citation.}\Danrui{Added}. 
But please note that our findings are derived from the comprehensive experimental results on all datasets with all time constraints. 


Table~\ref{tab:delta_acc_60} shows the results on 10 datasets within 60 seconds constraint. Each cell value represents the validation accuracy improvement using a particular search algorithm. For example, the first cell ``+3.07'' indicates that after 60 seconds, RS finds a preprocessing pipeline such that once it is applied, the validation accuracy gets improved by 3.07. This cell value is highlighted in bold because it is the highest value in the first row, meaning RS is the best search algorithm on the Australian dataset when the downstream model is LR. If a cell value equals to zero, it means that after 60 seconds, the corresponding search algorithm fails to find a preprocessing pipeline that can improve the model accuracy. 

We have two observations based on  Table~\ref{tab:delta_acc_60}. 

\textbf{1. Even with a short time limit, search algorithms can enhance the validation accuracy in most cases.} By looking at each individual column in Table \ref{tab:delta_acc_60}, we can see that most columns only have 1 or 2 zero values, indicating that the corresponding search algorithms can enhance the model accuracy in most cases. For example, the \textit{PBT} column only has a single zero value (i.e., when the dataset is \textit{Wine} and the downstream model is XGB). For all the other cases, the improvement is between 0.14 and 12.30. 

%most values are non-zero. For example, RS, Anneal, TPE, SMAC, TEVO\_Y, PBT, PMNE, PME, PLNE shows the significant short in a short time limit on all 10 datasets with all kinds of classifiers. For LR model, these search algorithms give improvement between 0.00 and 16.32 percent. For XGB model, the improvement is between 0.00 and 9.95 percent. And for MLP model, the improvemtn is between 0.00 and 44.55 percent.

\textbf{2. The degrees of improvement are different on different downstream models.} We can see that the degrees of improvement for LR and MLP are higher than XGB. For example, on the Forex dataset, when the search algorithm is \textit{RS}, the improvements for LR, XGB, MLP are 13.50, 5.79, 7.93, respectively. The LR is a linear model, which is hard to split different classes explicitly when data is more complex. It is sensitive to data changes like linear feature preprocessing. Thus the feature preprocessing can help it a lot.
%to get at lease 1.2 percent improvement. 
Tree models are not sensitive to the linear preprocessors like \textit{MinMaxScaler}. 
%Thus some non-linear operators like \textit{PowerTransformer} are more effective for improving XGB model.
Hence, under the same time limit, it is  harder to find an effective feature preprocessing pipeline for XGB model compared with LR model. MLP is also sensitive to data changes like LR, so we see big improvements for it. 

Next, we use \textit{RS} as a baseline and compare other search algorithms with it. Specifically, we compute the accuracy gap between each search algorithm and \textit{RS}. A positive (negative) gap implies that  \textit{RS} is better (worse). Due to the space constraint, we report the results on \textit{Australian} and \textit{Pd} datasets under 60s and 3600s time limits in Figure~\ref{fig:bar_vary_time_aus_pd}. We use "X" to represent the algorithms which cannot finish one complete evaluation. 


%In these experiments, we also find that \textit{RS} is still strong baseline. Thus, we exhibit the accuracy gap between \textit{RS} and other algorithms. Because of space limitation, we just exhibit the results with 60 and 3600 seconds time limit on \textit{Australian} and \textit{Pd} in Figure~\ref{fig:bar_vary_time_aus_pd}. We use "X" to express algorithms which cannot complete at least one complete evaluation. From Figure~\ref{fig:bar_vary_time_aus_pd}, we can get following insights:


%Based on Figure~\ref{fig:bar_vary_time_aus_pd}, get conclusion 1, 2 and 3, 4. Based on Figure~\ref{fig:ranking}, get conclusion 5.

\begin{table*}[htbp] 
\vspace{-5em} % h asks to places the floating element [h]ere.
  \caption{Validation accuracy improvement using different search algorithms on 10 datasets under 60 seconds time constrain.}
  \vspace{-.5em}
  \label{tab:delta_acc_60}
  \footnotesize
  \begin{tabular}{|p{0.06\textwidth}<{\centering}
                  |p{0.034\textwidth}<{\centering}
                  |p{0.03\textwidth}<{\centering}
                  p{0.034\textwidth}<{\centering}
                  p{0.03\textwidth}<{\centering}
                  p{0.034\textwidth}<{\centering}
                  p{0.045\textwidth}<{\centering}
                  p{0.04\textwidth}<{\centering}
                  p{0.032\textwidth}<{\centering}
                  p{0.07\textwidth}<{\centering}
                  p{0.034\textwidth}<{\centering}
                  p{0.08\textwidth}<{\centering}
                  p{0.035\textwidth}<{\centering}
                  p{0.03\textwidth}<{\centering}
                  p{0.03\textwidth}<{\centering}
                  p{0.03\textwidth}<{\centering}
                  p{0.035\textwidth}<{\centering}|}
    \hline
    \textbf{Dataset} & \textbf{ML Model} & \textbf{RS} & \textbf{Anneal} & \textbf{TPE} & \textbf{SMAC} & \textbf{TEVO\_H} & \textbf{TEVO\_Y} & \textbf{PBT} & \textbf{REINFORCE} & \textbf{ENAS} & \textbf{HYPERBAND} & \textbf{BOHB} & \textbf{PMNE} & \textbf{PME} & \textbf{PLNE} & \textbf{PLE} \\
    \hline
               & LR & \textbf{+3.07} & +1.81 & +1.81 & +1.81 & +2.35 & +2.71 & +2.53 & +2.89 & +2.35 & +1.99 & +1.45 & +1.99 & +1.99 & +1.27 & +0.91\\
    Australian & XGB & +3.21 & +2.49 & +2.85 & +2.85 & +3.75 & \textbf{+3.93} & +3.75 & +2.85 & +1.59 & +2.67 & +0.51 & +2.85 & +2.85 & +1.05 & +0.00\\
               & MLP & +5.15 & +4.97 & +4.43 & +3.89 & \textbf{+5.69} & \textbf{+5.69} & +5.15 & +4.07 & +3.53 & +3.89 & +3.89 & +4.07 & +4.07 & +4.43 & +3.89\\
    \hline
          & LR & +3.50 & +3.33 & +3.33 & +3.33 & +4.00 & +4.00 & \textbf{+4.17} & +2.83 & +1.67 & +3.50 & +2.33 & +3.33 & +3.33 & +3.33 & +3.33 \\
    Blood & XGB & +8.29 & +6.95 & +7.79 & +6.95 & +8.95 & +8.79 & \textbf{+9.95} & +8.45 & +7.62 & +8.29 & +7.62 & +8.62 & +8.62 & +6.79 & +5.62\\
          & MLP & +6.78 & +6.78 & +6.61 & \textbf{+7.28} & +6.95 & +6.95 & \textbf{+7.28} & +5.45 & +5.61 & +6.45 & +6.45 & \textbf{+7.28} & \textbf{+7.28} & +6.45 & +6.45\\
    \hline
            & LR & +10.16 & +9.21 & +8.26 & +9.53 & +9.21 & +8.58 & +10.48 & \textbf{+11.12} & +8.58 & +8.26 & +6.99 & +7.62 & +7.62 & +7.94 & +6.35\\
    Emotion & XGB & +0.42 & +0.1 & +0.42 & +0.74 & +1.05 & +0.42 & +0.42 & \textbf{+1.37} & +0.00 & +0.10 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00\\
            & MLP & +44.23 & +43.92 & \textbf{+44.55} & +43.60 & +43.92 & +43.92 & +43.92 & +42.96 & +43.28 & +42.96 & +43.60 & +43.92 & +43.6 & +44.23 & +41.69\\
    \hline
          & LR & +13.50 & \textbf{+16.32} & +14.79 & +12.97 & +14.67 & +14.15 & +13.12 & +10.87 & +10.73 & +0.00 & +0.00 & +11.94 & +11.16 & +10.00 & +9.98\\
    Forex & XGB & +5.79 & +5.85 & +3.60 & +3.73 & +4.85 & +4.85 & \textbf{+9.32} & +0.00 & +0.00 & +0.00 & +0.00 & +0.09 & +0.09 & +2.27 & +0.09\\
          & MLP & +7.93 & +3.23 & +3.28 & +0.72 & +5.76 & +5.76 & \textbf{+7.24} & +0.00 & +0.00 & +0.00 & +0.00 & +0.81 & +0.81 & +0.78 & +0.78\\
    \hline
          & LR & +6.12 & +4.08 & +4.49 & +6.12 & \textbf{+7.35} & \textbf{+7.35} & +5.31 & +5.72 & +4.08 & +4.49 & +3.27 & +6.12 & +6.12 & +2.45 & +0.41\\
    Heart & XGB & +3.84 & +0.16 & +0.16 & +2.20 & +2.61 & +3.02 & \textbf{+3.84} & +0.98 & +0.00 & +0.57 & +0.00 & +2.20 & +2.20 & +0.00 & +0.00\\
          & MLP & +26.94 & +26.13 & +27.76 & +26.53 & +27.76 & +27.76 & +27.35 & \textbf{+28.17} & +25.31 & +25.72 & +24.90 & +25.31 & +26.13 & +26.13 & +24.49\\
    \hline
            & LR & +2.85 & +2.94 & +2.89 & +2.73 & +2.89 & +2.89 & +2.85 & \textbf{+3.02} & +2.98 & +0.00 & +0.00 & +2.73 & +2.73 & +2.81 & +2.73\\
    Jasmine & XGB & +1.34 & +1.09 & +1.25 & +0.92 & \textbf{+1.38} & \textbf{+1.38} & +1.30 & +0.33 & +0.38 & +0.00 & +0.00 & +1.09 & +1.30 & +1.09 & +1.00\\
            & MLP & +1.73 & +1.69 & +2.32 & +2.23 & +1.90 & +1.90 & +2.07 & +1.23 & +1.82 & +0.00 & +0.00 & \textbf{+2.23} & \textbf{+2.23} & \textbf{+2.23} & \textbf{+2.23}\\
    \hline
             & LR & +4.86 & +5.17 & +4.86 & +2.99 & \textbf{+5.49} & \textbf{+5.49} & +5.29 & +3.66 & +3.15 & +0.00 & +0.00 & +4.98 & +4.98 & +4.06 & +3.39\\
    Madeline& XGB & +0.10 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.14 & +0.00 & +0.00 & +0.00 & +0.00 & \textbf{+0.62} & \textbf{+0.62} & \textbf{+0.62} & \textbf{+0.62}\\
             & MLP & +12.30 & +11.46 & +11.78 & +13.25 & +9.99 & +10.39 & +12.30 & +8.52 & +7.37 & +0.00 & +0.00 & +13.85 & +13.85 & \textbf{+14.13} & +13.85\\
    \hline
                         & LR & +11.14 & +10.98 & +11.14 & +11.8 & +11.31 & +11.64 & \textbf{+11.97} & +1.55 & +6.18 & +0.00 & +0.00 & +11.80 & +11.80 & +11.80 & +11.80\\
    Pd & XGB & +2.37 & +2.70 & +2.37 & +1.88 & +2.37 & +2.37 & \textbf{+3.03} & +0.00 & +0.00 & +0.00 & +0.00 & +2.21 & +1.88 & +1.88 & +2.37\\
                         & MLP & +19.94 & +19.44 & +21.09 & +19.44 & +21.43 & +21.43 & +20.93 & +6.88 & +15.48 & +0.00 & +0.00 & +21.92 & +21.92 & \textbf{+22.25} & \textbf{+22.25}\\
    \hline
                  & LR & +8.38 & +8.37 & +8.25 & \textbf{+9.13} & +8.04 & +8.42 & +8.13 & +8.46 & +6.52 & +8.38 & +8.17 & +7.96 & +7.94 & +8.29 & +7.88\\
    Wine & XGB & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00 & +0.00\\
                  & MLP & +7.75 & +4.92 & +7.13 & \textbf{+8.15} & +7.17 & +7.17 & +7.48 & +0.00 & +0.92 & +0.00 & +0.00 & \textbf{+8.15} & \textbf{+8.15} & \textbf{+8.15} & \textbf{+8.15}\\
    \hline
                      & LR & +6.70 & +6.56 & +6.88 & +6.03 & +7.05 & +7.05 & \textbf{+7.28} & +6.07 & +5.80 & +6.56 & +6.12 & +6.92 & +6.65 & +6.07 & +6.03\\
    Thyroid & XGB & +1.09 & +1.58 & +2.21 & \textbf{+2.88} & +2.38 & +2.38 & +2.43 & +0.00 & +0.00 & +0.51 & +0.42 & +1.27 & +1.18 & +1.63 & +0.64\\
                      & MLP & +4.91 & +4.60 & +4.73 & \textbf{+5.76} & +4.82 & +4.82 & +5.45 & +1.47 & +2.23 & +0.00 & +0.00 & +5.09 & +5.09 & +5.09 & +5.09\\
  \hline
\end{tabular}
\end{table*}


\iffalse
\begin{table*}[htbp] 
\vspace{-1em} % h asks to places the floating element [h]ere.
  \caption{Validation accuracy improvement using different search algorithms on 10 datasets under 60 seconds time constrain.}
  \vspace{-.5em}
  \label{tab:delta_acc_60}
  \footnotesize
  \begin{tabular}{|p{0.06\textwidth}<{\centering}
                  |p{0.034\textwidth}<{\centering}
                  |p{0.03\textwidth}<{\centering}
                  p{0.034\textwidth}<{\centering}
                  p{0.03\textwidth}<{\centering}
                  p{0.034\textwidth}<{\centering}
                  p{0.045\textwidth}<{\centering}
                  p{0.04\textwidth}<{\centering}
                  p{0.032\textwidth}<{\centering}
                  p{0.07\textwidth}<{\centering}
                  p{0.034\textwidth}<{\centering}
                  p{0.08\textwidth}<{\centering}
                  p{0.035\textwidth}<{\centering}
                  p{0.03\textwidth}<{\centering}
                  p{0.03\textwidth}<{\centering}
                  p{0.03\textwidth}<{\centering}
                  p{0.035\textwidth}<{\centering}|}
    \hline
    \textbf{Dataset} & \textbf{ML Model} & \textbf{RS} & \textbf{Anneal} & \textbf{TPE} & \textbf{SMAC} & \textbf{TEVO\_H} & \textbf{TEVO\_Y} & \textbf{PBT} & \textbf{REINFORCE} & \textbf{ENAS} & \textbf{HYPERBAND} & \textbf{BOHB} & \textbf{PMNE} & \textbf{PME} & \textbf{PLNE} & \textbf{PLE} \\
  \hline
	& LR & 1.33 & 1.39 & 1.2 & 0.75 & 1.6 & \textbf{1.72} & \textbf{1.72} & 0.69 & 0.0 & 0.0 & 0.0 & 1.66 & 1.66 & 0.45 & 0.45\\
	Ada 	& XGB & 0.72 & 0.36 & 0.36 & \textbf{0.9} & 0.54 & 0.54 & 0.42 & 0.0 & 0.0 & 0.0 & 0.0 & 0.6 & 0.6 & 0.3 & 0.3\\
	& MLP & 11.02 & 10.93 & 11.3 & 10.84 & 10.78 & 10.78 & 11.2 & 9.22 & 8.83 & 0.0 & 0.0 & \textbf{11.57} & 11.3 & 11.36 & 11.36\\
\hline
	& LR & \textbf{3.06} & 1.8 & 1.8 & 1.8 & 2.34 & 2.7 & 2.52 & 2.88 & 2.34 & 1.98 & 1.44 & 1.98 & 1.98 & 1.26 & 0.9\\
	Austrilian 	& XGB & 3.96 & 3.24 & 3.6 & 3.6 & 4.5 & \textbf{4.68} & 4.5 & 3.6 & 2.34 & 3.42 & 1.26 & 3.6 & 3.6 & 1.8 & 0.0\\
	& MLP & 11.17 & 10.99 & 10.45 & 9.91 & \textbf{11.71} & \textbf{11.71} & 11.17 & 10.09 & 9.55 & 9.91 & 9.91 & 10.09 & 10.09 & 10.45 & 9.91\\
\hline
	& LR & 3.5 & 3.33 & 3.33 & 3.33 & 4.0 & 4.0 & \textbf{4.17} & 2.83 & 1.67 & 3.5 & 2.33 & 3.33 & 3.33 & 3.33 & 3.33\\
	Blood 	& XGB & 4.67 & 3.33 & 4.17 & 3.33 & 5.33 & 5.17 & \textbf{6.33} & 4.83 & 4.0 & 4.67 & 4.0 & 5.0 & 5.0 & 3.17 & 2.0\\
	& MLP & 2.0 & 2.0 & 1.83 & \textbf{2.5} & 2.17 & 2.17 & \textbf{2.5} & 0.67 & 0.83 & 1.67 & 1.67 & \textbf{2.5} & \textbf{2.5} & 1.67 & 1.67\\
\hline
	& LR & 0.0 & 0.53 & 0.0 & 1.15 & 0.53 & 0.53 & 1.64 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{2.65} & \textbf{2.65} & \textbf{2.65} & \textbf{2.65}\\
	Christine 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 0.0 & 2.38 & 2.38 & 2.88 & 2.51 & 3.88 & 5.42 & 1.15 & 0.0 & 0.0 & 0.0 & \textbf{9.34} & \textbf{9.34} & \textbf{9.34} & \textbf{9.34}\\
\hline
	& LR & 0.14 & 0.13 & 0.11 & 0.08 & \textbf{0.21} & \textbf{0.21} & 0.2 & 0.1 & 0.11 & 0.0 & 0.0 & 0.11 & 0.14 & 0.08 & 0.08\\
	Click\_Prediction\_Small 	& XGB & 0.0 & 0.0 & 0.0 & \textbf{0.02} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{0.02} & \textbf{0.02} & \textbf{0.02} & \textbf{0.02}\\
	& MLP & 0.22 & 0.2 & 0.0 & 0.0 & 0.11 & 0.11 & 0.16 & 0.01 & 0.01 & 0.0 & 0.0 & \textbf{0.39} & \textbf{0.39} & \textbf{0.39} & \textbf{0.39}\\
\hline
	& LR & 3.43 & 3.31 & 3.43 & \textbf{3.46} & \textbf{3.46} & \textbf{3.46} & 3.43 & 3.1 & 2.93 & 0.0 & 0.0 & \textbf{3.46} & \textbf{3.46} & \textbf{3.46} & \textbf{3.46}\\
	Credit 	& XGB & \textbf{0.05} & 0.0 & \textbf{0.05} & 0.01 & 0.0 & 0.0 & 0.01 & 0.0 & 0.0 & 0.0 & 0.0 & 0.02 & 0.02 & 0.02 & 0.02\\
	& MLP & \textbf{3.44} & 2.12 & 0.28 & 0.0 & 2.7 & 2.7 & 3.11 & 1.1 & 0.72 & 0.0 & 0.0 & 3.13 & 3.13 & 3.13 & 3.13\\
\hline
	& LR & 3.92 & 3.3 & 3.8 & \textbf{4.11} & 3.61 & 3.6 & 1.99 & 3.17 & 2.75 & 0.0 & 0.0 & 3.64 & 3.75 & 0.84 & 0.74\\
	Eeg 	& XGB & 0.04 & \textbf{0.05} & 0.04 & 0.04 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.04 & 0.04 & 0.04 & 0.04\\
	& MLP & \textbf{36.65} & 20.71 & 36.1 & 15.81 & 33.23 & 33.23 & 34.79 & 6.42 & 18.19 & 0.0 & 0.0 & 30.16 & 31.1 & 34.84 & 34.84\\
\hline
	& LR & 0.83 & 0.79 & 0.76 & \textbf{1.16} & 0.68 & 0.68 & 0.79 & 0.31 & 0.79 & 0.0 & 0.0 & 0.79 & 0.77 & 0.76 & 0.76\\
	Electricity 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.36 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{3.01} & \textbf{3.01} & \textbf{3.01} & \textbf{3.01}\\
\hline
	& LR & 8.57 & 7.62 & 6.67 & 7.94 & 7.62 & 6.98 & 8.89 & \textbf{9.52} & 6.98 & 6.67 & 5.4 & 6.03 & 6.03 & 6.35 & 4.76\\
	Emotion 	& XGB & 9.21 & 8.89 & 9.21 & 9.52 & 9.84 & 9.21 & 9.21 & \textbf{10.16} & 8.25 & 8.89 & 8.25 & 7.3 & 7.3 & 7.62 & 6.35\\
	& MLP & 5.4 & 5.08 & \textbf{5.71} & 4.76 & 5.08 & 5.08 & 5.08 & 4.13 & 4.44 & 4.13 & 4.76 & 5.08 & 4.76 & 5.4 & 2.86\\
\hline
	& LR & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{0.15} & \textbf{0.15} & \textbf{0.15} & \textbf{0.15}\\
	Fibert 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & 13.49 & \textbf{16.31} & 14.78 & 12.96 & 14.66 & 14.14 & 13.11 & 10.86 & 10.72 & 0.0 & 0.0 & 11.93 & 11.15 & 9.99 & 9.97\\
	Forex 	& XGB & 5.71 & 5.77 & 3.52 & 3.65 & 4.77 & 4.77 & \textbf{9.25} & 0.0 & 0.0 & 0.0 & 0.0 & 0.01 & 0.01 & 2.2 & 0.01\\
	& MLP & \textbf{12.2} & 7.5 & 7.55 & 4.99 & 10.03 & 10.03 & 11.5 & 3.33 & 4.05 & 0.0 & 0.0 & 5.08 & 5.05 & 5.05 & 5.05\\
\hline
	& LR & \textbf{5.56} & 5.44 & 5.44 & 5.51 & 4.49 & 4.49 & 4.56 & 5.05 & 4.52 & 0.0 & 0.0 & 5.49 & 5.49 & 5.38 & 5.39\\
	Gesture 	& XGB & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{0.25} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
	& MLP & 4.15 & 2.62 & \textbf{5.84} & 5.44 & 1.43 & 4.29 & 5.44 & 0.0 & 0.0 & 0.0 & 0.0 & 5.25 & 5.25 & 5.25 & 5.25\\
\hline
	& LR & 8.16 & 6.12 & 6.53 & 8.16 & \textbf{9.39} & \textbf{9.39} & 7.35 & 7.76 & 6.12 & 6.53 & 5.31 & 8.16 & 8.16 & 4.49 & 2.45\\
	Heart 	& XGB & \textbf{9.8} & 6.12 & 6.12 & 8.16 & 8.57 & 8.98 & \textbf{9.8} & 6.94 & 4.9 & 6.53 & 3.67 & 8.16 & 8.16 & 4.08 & 0.41\\
	& MLP & 14.69 & 13.88 & 15.51 & 14.29 & 15.51 & 15.51 & 15.1 & \textbf{15.92} & 13.06 & 13.47 & 12.65 & 13.06 & 13.88 & 13.88 & 12.24\\
\hline
	& LR & 2.97 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{8.35} & \textbf{8.35} & \textbf{8.35} & \textbf{8.35}\\
	Helena 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & 0.0 & 0.0 & 0.08 & \textbf{0.22} & 0.0 & 0.0 & 0.08 & 0.0 & 0.0 & 0.0 & 0.0 & 0.2 & 0.15 & 0.15 & 0.15\\
	Higgs 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & 17.0 & 17.17 & 16.71 & 16.51 & 16.48 & 16.48 & 17.02 & 7.91 & 10.19 & 0.0 & 0.0 & 16.88 & \textbf{17.19} & 16.51 & 16.51\\
	House\_Data 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 52.22 & 38.71 & 45.55 & 25.7 & 43.11 & 41.0 & 52.91 & 36.36 & 27.49 & 0.0 & 0.0 & \textbf{53.9} & \textbf{53.9} & \textbf{53.9} & \textbf{53.9}\\
\hline
	& LR & 4.01 & 2.92 & 2.16 & 4.3 & 3.95 & 3.95 & 4.19 & 0.0 & 0.5 & 0.0 & 0.0 & 4.34 & 4.34 & 4.34 & \textbf{4.35}\\
	Jannis 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & 2.85 & 2.93 & 2.89 & 2.72 & 2.89 & 2.89 & 2.85 & \textbf{3.01} & 2.97 & 0.0 & 0.0 & 2.72 & 2.72 & 2.8 & 2.72\\
	Jasmine 	& XGB & 1.46 & 1.21 & 1.38 & 1.05 & \textbf{1.51} & \textbf{1.51} & 1.42 & 0.46 & 0.5 & 0.0 & 0.0 & 1.21 & 1.42 & 1.21 & 1.13\\
	& MLP & 2.64 & 2.59 & \textbf{3.22} & 3.14 & 2.8 & 2.8 & 2.97 & 2.13 & 2.72 & 0.0 & 0.0 & 3.14 & 3.14 & 3.14 & 3.14\\
\hline
	& LR & 0.77 & 0.47 & 0.83 & 0.59 & 0.83 & \textbf{1.07} & 0.89 & 0.53 & 0.24 & 0.65 & 0.53 & 0.71 & 0.71 & 0.59 & 0.59\\
	Kc1 	& XGB & 1.48 & 1.48 & 1.48 & 1.54 & \textbf{1.78} & \textbf{1.78} & 1.66 & 1.18 & 0.0 & 1.42 & 1.18 & \textbf{1.78} & \textbf{1.78} & 1.12 & 0.89\\
	& MLP & 6.69 & \textbf{7.46} & 6.86 & 6.21 & 7.04 & 7.04 & 6.86 & 4.08 & 4.73 & 6.57 & 6.51 & 6.69 & 6.57 & 6.63 & 6.51\\
\hline
	& LR & 4.25 & 4.57 & 4.25 & 2.39 & \textbf{4.89} & \textbf{4.89} & 4.69 & 3.06 & 2.54 & 0.0 & 0.0 & 4.37 & 4.37 & 3.46 & 2.78\\
	Madeline 	& XGB & 1.07 & 0.0 & 0.64 & 0.0 & 0.83 & 0.83 & 1.11 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{1.59} & \textbf{1.59} & \textbf{1.59} & \textbf{1.59}\\
	& MLP & 5.61 & 4.77 & 5.09 & 6.56 & 3.3 & 3.7 & 5.61 & 1.83 & 0.68 & 0.0 & 0.0 & 7.16 & 7.16 & \textbf{7.44} & 7.16\\
\hline
	& LR & \textbf{0.14} & 0.0 & 0.07 & 0.04 & 0.03 & 0.03 & 0.06 & 0.0 & 0.0 & 0.0 & 0.0 & 0.02 & 0.02 & 0.01 & 0.01\\
	Numerai28.6 	& XGB & 0.0 & 0.03 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{0.06} & 0.0 & 0.0 & 0.0 & 0.0 & 0.04 & 0.04 & 0.04 & 0.04\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & 11.74 & 11.57 & 11.74 & 12.4 & 11.9 & 12.23 & \textbf{12.56} & 2.15 & 6.78 & 0.0 & 0.0 & 12.4 & 12.4 & 12.4 & 12.4\\
	Pd\_Speech\_Features 	& XGB & 0.5 & 0.83 & 0.5 & 0.0 & 0.5 & 0.5 & \textbf{1.16} & 0.0 & 0.0 & 0.0 & 0.0 & 0.33 & 0.0 & 0.0 & 0.5\\
	& MLP & 69.09 & 68.6 & 70.25 & 68.6 & 70.58 & 70.58 & 70.08 & 56.03 & 64.63 & 0.0 & 0.0 & 71.07 & 71.07 & \textbf{71.4} & \textbf{71.4}\\
\hline
	& LR & 2.38 & 2.14 & 2.04 & \textbf{2.68} & 2.17 & 2.32 & 2.42 & 0.0 & 0.0 & 0.0 & 0.0 & 2.57 & 2.57 & 2.59 & 2.59\\
	Philippine 	& XGB & 0.04 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{0.17} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0\\
	& MLP & 20.51 & 15.78 & 17.15 & 20.9 & 18.37 & 21.18 & \textbf{21.44} & 17.34 & 14.15 & 0.0 & 0.0 & 21.11 & 21.11 & 21.33 & 21.33\\
\hline
	& LR & 2.68 & 2.36 & 2.2 & 2.54 & 2.54 & 2.73 & 2.73 & \textbf{2.91} & 2.06 & 2.38 & 2.01 & 2.82 & 2.54 & 1.39 & 0.81\\
	Phoneme 	& XGB & 0.67 & 0.39 & 0.44 & 0.25 & 0.46 & 0.53 & 0.46 & 0.55 & 0.42 & 0.42 & 0.39 & \textbf{0.81} & \textbf{0.81} & 0.46 & 0.12\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & 6.7 & 6.56 & 6.88 & 6.03 & 7.05 & 7.05 & \textbf{7.28} & 6.07 & 5.8 & 6.56 & 6.12 & 6.92 & 6.65 & 6.07 & 6.03\\
	Thyroid-Allhyper 	& XGB & 0.45 & 0.94 & 1.56 & \textbf{2.23} & 1.74 & 1.74 & 1.79 & 0.0 & 0.0 & 0.0 & 0.0 & 0.63 & 0.54 & 0.98 & 0.0\\
	& MLP & 4.29 & 3.97 & 4.11 & \textbf{5.13} & 4.2 & 4.2 & 4.82 & 0.85 & 1.61 & 0.0 & 0.0 & 4.46 & 4.46 & 4.46 & 4.46\\
\hline
	& LR & 6.32 & 6.18 & 6.18 & 6.62 & 6.62 & \textbf{7.5} & 6.32 & 6.62 & 5.44 & 6.03 & 5.88 & 6.62 & 6.62 & 5.88 & 5.88\\
	Vehicle 	& XGB & 3.53 & 2.79 & 3.38 & \textbf{4.41} & 3.68 & 3.68 & 3.97 & 3.38 & 0.0 & 3.38 & 3.09 & \textbf{4.41} & \textbf{4.41} & 2.21 & 2.21\\
	& MLP & \textbf{19.85} & \textbf{19.85} & \textbf{19.85} & \textbf{19.85} & \textbf{19.85} & \textbf{19.85} & 19.56 & 17.5 & 18.82 & 18.68 & 18.82 & \textbf{19.85} & \textbf{19.85} & \textbf{19.85} & \textbf{19.85}\\
\hline
	& LR & 3.74 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.06 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{4.51} & \textbf{4.51} & \textbf{4.51} & \textbf{4.51}\\
	Volkert 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & 8.96 & 8.94 & 8.83 & \textbf{9.71} & 8.62 & 9.0 & 8.71 & 9.04 & 7.1 & 8.96 & 8.75 & 8.54 & 8.52 & 8.87 & 8.46\\
	Wine\_Quality 	& XGB & 0.21 & 0.1 & 0.21 & 0.29 & 0.27 & 0.27 & 0.19 & 0.0 & 0.0 & \textbf{0.33} & \textbf{0.33} & 0.29 & 0.29 & 0.31 & 0.29\\
	& MLP & 7.19 & 4.37 & 6.58 & \textbf{7.6} & 6.62 & 6.62 & 6.92 & 0.0 & 0.37 & 0.0 & 0.0 & \textbf{7.6} & \textbf{7.6} & \textbf{7.6} & \textbf{7.6}\\
\hline
	& LR & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48} & \textbf{1.48}\\
	Analcatdata\_Authorship 	& XGB & \textbf{0.89} & 0.74 & 0.74 & 0.74 & 0.74 & 0.74 & 0.74 & 0.59 & 0.44 & 0.59 & 0.0 & 0.74 & 0.74 & 0.74 & 0.74\\
	& MLP & \textbf{2.96} & \textbf{2.96} & \textbf{2.96} & \textbf{2.96} & \textbf{2.96} & \textbf{2.96} & \textbf{2.96} & \textbf{2.96} & 2.81 & 2.81 & 0.0 & \textbf{2.96} & \textbf{2.96} & \textbf{2.96} & \textbf{2.96}\\
\hline
	& LR & 4.67 & 4.73 & 4.59 & \textbf{4.85} & 4.21 & 4.21 & 4.73 & 0.0 & 0.04 & 0.0 & 0.0 & \textbf{4.85} & \textbf{4.85} & \textbf{4.85} & \textbf{4.85}\\
	Gas-Drift 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 3.21 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{3.3} & 0.0 & 0.0 & 0.0 & 0.0 & 3.19 & 3.19 & 3.19 & 3.19\\
\hline
	& LR & 0.0 & 0.0 & 0.0 & \textbf{0.18} & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{0.18} & \textbf{0.18} & \textbf{0.18} & \textbf{0.18}\\
	Har 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{0.36} & \textbf{0.36} & \textbf{0.36} & \textbf{0.36}\\
\hline
	& LR & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	Hill 	& XGB & \textbf{45.88} & \textbf{45.88} & \textbf{45.88} & \textbf{45.88} & \textbf{45.88} & \textbf{45.88} & \textbf{45.88} & 45.77 & \textbf{45.88} & 0.0 & 0.0 & \textbf{45.88} & \textbf{45.88} & \textbf{45.88} & \textbf{45.88}\\
	& MLP & 45.67 & 42.89 & 44.85 & \textbf{46.39} & 44.33 & 44.33 & 44.23 & 46.08 & 24.02 & 0.0 & 0.0 & \textbf{46.39} & \textbf{46.39} & 44.12 & 40.82\\
\hline
	& LR & 7.14 & 6.43 & 6.43 & 5.36 & \textbf{7.5} & \textbf{7.5} & \textbf{7.5} & 6.79 & 4.64 & 6.43 & 6.07 & 7.14 & 7.14 & 4.64 & 3.57\\
	Ionosphere 	& XGB & 8.57 & 7.5 & 7.5 & 7.14 & 8.93 & \textbf{9.29} & 8.21 & \textbf{9.29} & 4.64 & 8.21 & 7.5 & 7.86 & 7.86 & 5.36 & 2.14\\
	& MLP & 3.93 & \textbf{5.0} & \textbf{5.0} & 3.57 & 3.93 & 3.57 & \textbf{5.0} & 2.5 & 2.5 & 3.57 & 4.64 & 3.57 & 3.57 & 3.57 & 3.57\\
\hline
	& LR & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	Isolet 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & \textbf{35.31} & \textbf{35.31} & \textbf{35.31} & \textbf{35.31} & \textbf{35.31} & \textbf{35.31} & \textbf{35.31} & 32.13 & 34.0 & \textbf{35.31} & \textbf{35.31} & \textbf{35.31} & \textbf{35.31} & \textbf{35.31} & \textbf{35.31}\\
	Mobile\_Price 	& XGB & 2.19 & 2.12 & 2.69 & \textbf{2.81} & 2.69 & 2.69 & 2.62 & 1.0 & 0.0 & 1.94 & 0.37 & 2.25 & 2.19 & 1.63 & 1.56\\
	& MLP & 32.56 & 32.69 & 32.69 & 32.81 & \textbf{33.06} & \textbf{33.06} & 33.0 & 22.81 & 25.31 & 31.25 & 12.5 & 32.81 & 32.81 & 32.81 & 32.81\\
\hline
	& LR & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56} & \textbf{7.56}\\
	Mozilla4 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{1.0} & 0.99 & 0.75 & \textbf{1.0} & 0.96 & 0.96 & 0.96 & 0.96 & 0.68 & 0.0 & 0.0 & 0.96 & 0.96 & 0.96 & 0.96\\
\hline
	& LR & 14.51 & 14.61 & \textbf{15.65} & 15.47 & 15.09 & 15.31 & 14.99 & 14.77 & 14.4 & 0.0 & 0.0 & 14.27 & 13.81 & 12.53 & 13.09\\
	Nasa 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{81.63} & 81.55 & 81.31 & 81.07 & \textbf{81.63} & \textbf{81.63} & 81.39 & 79.76 & 78.21 & 0.0 & 0.0 & 81.15 & 81.07 & 81.25 & 81.07\\
\hline
	& LR & 2.21 & 2.31 & 2.37 & 2.17 & \textbf{2.67} & \textbf{2.67} & 2.53 & 2.1 & 0.98 & 2.01 & 1.87 & 2.63 & 2.63 & 1.83 & 1.83\\
	Page 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 0.57 & \textbf{0.59} & 0.43 & 0.34 & 0.57 & 0.57 & 0.53 & 0.0 & 0.0 & 0.43 & 0.0 & 0.34 & 0.34 & 0.34 & 0.34\\
\hline
	& LR & 16.77 & 16.84 & 15.76 & 16.27 & 15.44 & 15.85 & 14.34 & 14.73 & 11.66 & 0.0 & 0.0 & \textbf{17.02} & \textbf{17.02} & 14.68 & 14.68\\
	Robot 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 4.08 & 3.0 & 3.32 & \textbf{4.58} & 3.73 & 3.41 & 3.83 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{4.58} & \textbf{4.58} & \textbf{4.58} & \textbf{4.58}\\
\hline
	& LR & 12.3 & 12.19 & 12.1 & \textbf{13.21} & 10.8 & 10.8 & 11.54 & 11.67 & 11.35 & 0.0 & 0.0 & 12.28 & 12.03 & 11.78 & 11.78\\
	Run\_Or\_Walk 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
	& LR & 1.68 & 1.6 & 1.68 & 1.63 & \textbf{1.82} & 1.79 & 1.77 & 1.01 & 0.95 & 0.0 & 0.0 & 1.71 & 1.74 & 1.63 & 1.63\\
	Spambase 	& XGB & 0.33 & 0.11 & 0.3 & \textbf{0.41} & 0.27 & 0.27 & 0.3 & 0.0 & 0.0 & 0.0 & 0.0 & 0.14 & 0.14 & 0.14 & 0.14\\
	& MLP & 2.36 & 2.2 & 2.2 & 2.31 & \textbf{2.58} & 2.55 & \textbf{2.58} & 1.44 & 1.49 & 0.0 & 0.0 & 2.31 & 2.31 & 2.31 & 2.31\\
\hline
	& LR & 8.12 & 7.95 & 8.0 & 8.05 & 8.2 & 8.2 & 8.17 & 8.0 & 8.17 & 7.9 & 0.0 & \textbf{8.22} & \textbf{8.22} & 7.8 & 7.8\\
	Sylvine 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 8.9 & 8.34 & 8.41 & \textbf{9.02} & 8.63 & 8.63 & 8.88 & 4.9 & 5.27 & 0.0 & 0.0 & \textbf{9.02} & \textbf{9.02} & \textbf{9.02} & \textbf{9.02}\\
\hline
	& LR & \textbf{17.04} & 16.88 & 15.76 & 16.27 & 16.82 & \textbf{17.04} & 15.12 & 16.27 & 13.86 & 0.0 & 0.0 & 17.02 & 16.95 & 14.68 & 14.68\\
	Wall-Robot 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & 3.53 & 2.59 & 2.38 & 3.55 & 3.02 & 3.02 & 2.79 & 0.0 & 0.0 & 0.0 & 0.0 & \textbf{3.71} & 3.6 & 3.64 & 3.64\\
\hline
	& LR & 1.26 & 1.16 & 1.24 & 1.42 & \textbf{1.57} & 1.47 & 1.37 & 1.03 & 0.05 & 1.14 & 0.0 & 1.32 & 1.32 & 1.03 & 1.03\\
	Wilt 	& XGB & 0.59 & 0.39 & 0.44 & 0.26 & \textbf{0.65} & \textbf{0.65} & 0.57 & 0.36 & 0.26 & 0.31 & 0.41 & \textbf{0.65} & \textbf{0.65} & 0.13 & 0.0\\
	& MLP & 1.08 & 1.08 & 1.08 & \textbf{1.16} & \textbf{1.16} & \textbf{1.16} & \textbf{1.16} & 0.0 & 0.0 & 0.54 & 0.83 & \textbf{1.16} & \textbf{1.16} & \textbf{1.16} & \textbf{1.16}\\
\hline
	& LR & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 0.0 & 2.45 & \textbf{4.09} & \textbf{4.09} & 2.45\\
	Covtype 	& XGB & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
	& MLP & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0} & \textbf{0.0}\\
\hline
\end{tabular}
\end{table*}
\fi




\begin{figure*}[h]
\vspace{-.5em}
\centering
\includegraphics[width=\textwidth]{figures/bar_vary_time_aus_pd.eps}
\vspace{-1.5em}
\caption{The gap of the validation accuracy of random search and other search algorithms on Australian and Pd datasets with 60s and 3600s time limits.}
\label{fig:bar_vary_time_aus_pd}
\end{figure*}


\textbf{3. There is no all-time winner.} Figure~\ref{fig:bar_vary_time_aus_pd} shows that if an algorithm achieves the best performance with a specific dataset, downstream model and time limit, when one of the three factors changes, the winner may not hold. For example, on the \textit{Australian} dataset with an XGB model and 60 seconds time limit, \textit{TEVO\_Y} shows the best performance. When the dataset is changed to \textit{Pd}, \textit{PBT} becomes the winner, although the two other factors (model and time limit) remain the same. 



\textbf{4. \textit{RS} is still a strong baseline.} We observe that most algorithms cannot outperform \textit{RS} by a lot. In many situations, they even performed worse. For example, in Figure~\ref{fig:bar_vary_time_aus_pd}, many algorithms have negative accuracy gaps w.r.t. \textit{RS}. For example, on \textit{Australian} dataset (LR), when the time limit is 60 seconds, none of algorithms outperform \textit{RS}; when the time limit is 3600 seconds, only \textit{PME} and \textit{PLNE} achieve better performance than \textit{RS}. %  surrogate-model-based \textit{SMAC}  performed better than \textit{RS} only with \textit{LR} on \textit{Pd} dataset, evolution-based \textit{TEVO\_Y} cannot outperform \textit{RS} by a large margin, and bandit-based \textit{BOHB} always lost to \textit{RS}. 

\vspace{.5em}

In the following, we divide search algorithms into three categories and compare each of them with \textit{RS} in detail.
\begin{itemize}
    \item Surrogate-model-based: \textit{TPE}, \textit{BOHB}, \textit{SMAC}, \textit{REINFORCE}, \textit{ENAS}, \textit{PMNE}, \textit{PME}, \textit{PLNE} and \textit{PLE}.
    \item Bandit-based: \textit{Hyperband} and \textit{BOHB}
    \item Evolution-based: \textit{TEVO\_H}, \textit{TEVO\_Y}, and \textit{PBT}
\end{itemize}


We first compare surrogate-model-based algorithms with \textit{RS}.

\textbf{5. Surrogate-model-based algorithms do not outperform \textit{RS} in most cases.} By examining the  performance of surrogate-model-based algorithms, we find that they do not outperform \textit{RS} in most cases. The goal of surrogate models is to direct the search direction for next steps through a model, thus the precise directing is important for the performance of surrogate-model-based algorithms. However, surrogate-model-based algorithms that need initialization do not have enough data to promise the initial directions or only start with randomness. For example, the starting points of \textit{PMNE} are just the 7 pipelines with only one preprocessor, and \textit{REINFORCE} starts with a random parameter matrix. Furthermore, the  fitting process of surrogate models is time consuming, which causes fewer number of  pipelines evaluated. For example, \textit{SMAC} needs to train a random forest, \textit{TPE} needs to fit many KDEs, and \textit{PNAS} needs to fit a MLP or LSTM. When running \textit{RS} on \textit{Australian} with \textit{LR}, we can get 1102 evaluated pipelines, while the number for \textit{SMAC} is only 270. This insight also inspires us that the search space of feature preprocessing pipelines is hard to learn by general surrogate models like random forest, KDE, MLP and LSTM, and there is still a space to improve surrogate models for Auto-FP scenario specially. 
%\jn{I didn't get this part: Thus within the same time limit, less time is used to evaluate candidate pipelines, which means the not enough training data of updating surrogate models. It is a vicious cycle.} \Danrui{I deleted the previous sentence and added new reason}
%\Danrui{We know that the training of surrogate model is time consuming. In short, more fitting time of surrogate model = less number of evaluations = more imprecise surrogate model}

\textbf{6. \textit{REINFORCE} and \textit{ENAS} do not perform well in most cases.} From Figure~\ref{fig:bar_vary_time_aus_pd}, it is obvious that \textit{REINFORCE} and \textit{ENAS} do not perform well, especially with short time limit. There are two reasons. Firstly, the initialization of surrogate models of \textit{REINFORCE} and \textit{ENAS} are by random, which can lead to a wrong direction at the starting stage with a high probability. Secondly, \textit{REINFORCE} and \textit{ENAS} employ the idea of stochastic gradient descent, which updates model parameters after only one evaluation, which means the improvement of surrogate models is a slow process with lots of iterations. With the increase of time limit, the surrogate models become more and more precise, i.e., have higher opportunity to produce better pipelines. 

\vspace{.25em}

We next compare bandit-based algorithms with \textit{RS}.


\textbf{7. Within a short time limit, bandit-based algorithms cannot complete one full evaluation.} There are two bandit-based algorithms: \textit{Hyperband} and \textit{BOHB}. They first identify the most promising pipeline among a set of candidate pipelines and then run a full evaluation of the pipeline. If the first step takes too long, they will not complete a full evaluation thus fail to report any result. For example, on the \textit{Pd} dataset, when the time limit is 60 seconds, \textit{Hyperband} and \textit{BOHB} fail to report any result no matter what the downstream ML model is. In our setting, there are about 100 pipelines in the Success Halving process, and the algorithms spend over 60 seconds to figure out the most promising pipeline. While decreasing the number of candidate pipelines can mitigate this issue, the downside is that they will lose their bandit characteristics and perform like \textit{RS}.

\textbf{8. \textit{Hyperband} and \textit{BOHB} do not outperform \textit{RS} in most cases.} From Figure~\ref{fig:bar_vary_time_aus_pd}, even when \textit{Hyperband} and \textit{BOHB} can complete one Successive Halving process, they still cannot outperform \textit{RS} in most cases. Their main early-stopping idea cannot work well for LR, XGB and MLP under our setting. Even we try many possibilities of the two important parameters $\eta$ and \texttt{min\_budget} (See Figure~\ref{fig:hyperband_vary_eta_and_budget}. Due to the space limit, we only exhibit the result of \textit{Jasmine} with \textit{LR} model), it is still hard to make the two algorithms exceeds \textit{RS}. Also, it is hard to determine which parameter is better with different algorithms and time limits. Clearly, how to improve \textit{Hyperband} and \textit{BOHB}, specially for Auto-FP scenario, still needs further exploration.
 
\begin{figure}[t]
\vspace{-4em}
\centering
\includegraphics[width=\columnwidth]{figures/hyperband_vary_eta_and_budget_all_in_one.eps}
\caption{Parameter adjustment for \textit{Hyperband} and \textit{BOHB}. The upper two vary $\eta$. The lower two vary \texttt{min\_budget}.
}
\label{fig:hyperband_vary_eta_and_budget}
\end{figure}

%From Figure~\ref{fig:bar_vary_time_aus_pd}, even when \textit{Hyperband} and \textit{BOHB} can complete one Successive Halving process, they still cannot outperform \textit{RS} in most cases. This is because their main early-stopping idea which works well for DNN cannot work well for LR, XGB and MLP with our setting. For DNNs like LeNet, the loss curve depicting the correspondence between epoch and loss does not fluctuate very drastically because one epoch includes many iterations. Thus the training of DNNs benefits more from the early-stopping strategy. We consider single iteration or estimator as the resource in our setting, \jn{Why did we do it in this way: ``consider single iteration or estimator''? What stopped us from adoptting the same idea as DNNs}, which causes the validation accuracy curves fluctuate drastically according to the number of training iterations or estimators. At the starting stage with 3-5 estimators or iterations, the ranking of pipelines is not similar with the ranking under 100 estimators or iterations. However, at the early stage, about 1/3 pipelines including strong ones are stopped. Thus we cannot benefit much from early-stopping. 

%For illustrating this, we draw the validation accuracy curves according to 
%Thus we can conclude that \textit{Band}-based problems do not fit for feature preprocessing pipeline search scenario well. However, in \textcolor{red}{previous paper}, \textit{Band}-based algorithms can perform well on tasks like training deep neural networks. The reason is that for DNNs like LeNet, the resource of \textit{Band}-based algorithms is epoch. The loss curve of DNNs increases more slowly and stable according to the number of epochs, which means their curve does not fluctuate very drastically. Thus the training of DNNs benefits more from the early stopping strategy of \textit{Band}-based algorithms than feature preprocessing pipeline search scenario. 

%In our scenario, the downstream models are not as complex as DNNs, which means actually their validation accuracy curves fluctuate drastically according to the number of training iterations or estimators. At the starting stage with 3-5 estimators or iterations, the ranking of pipelines is not similar with the ranking under 100 estimators or iterations. However, at the early stage, about 1/3 pipelines are stopped which include some strong pipelines. Thus we cannot benefit much from early-stopping because early-stopping can stop powerful pipelines wrongly in the early stage.

%\begin{itemize}
%    \item Comparing with \textit{RS}, surrogate-model-based and evolution-based algorithms cannot outperform or outperform a lot
%\end{itemize}

\vspace{.25em}

We finally compare evolution-based algorithms with \textit{RS}.

\textbf{9. Evolution-based algorithms  outperform \textit{RS} in most cases.} From Figure~\ref{fig:bar_vary_time_aus_pd}, we observe that in most cases, at least one of the evolution-based algorithms (\textit{TEVO\_H}, \textit{TEVO\_Y} and \textit{PBT}) outperforms \textit{RS}. This is because that they have more exploitation than \textit{RS}, which can produce promising search directions for next steps. For example, \textit{TEVO\_H} mutates the best pipeline of sampled pipelines from the population. Moreover, unlike other search algorithms, evolution-based algorithms require a small overhead to select the next pipeline since they just sample then mutate. This allows them to evaluate many more pipelines under the same budget.  % Note that evolution-based algorithms are actually stronger \textit{RS}, thus their improvement comparing with \textit{RS} are not giant. 



%\textbf{4. In most cases, band-based algorithms cannot complete at least one full-training.}

%\textbf{Evolution-based algorithms have higher opportunity to overcome \textit{RS}, while surrogate-model-based algorithms have higher opportunity to lose comparing with \textit{RS}}. We mentioned that there is no all-time winner previously. However, in practice, user still want a recommendation especially when they are not familiar with the dataset or downstream ML model. For solving this case, we consider general ranking of the 15 algorithms. With 10 datasets, 6 time limits and 3 downstream ML models, each algorithm is tested on totally 180 scenarios. We rank them in each scenario by validation accuracy and converge time. Then we rank the average ranking of each algorithm throughout all 180 scenarios, which is shown in Figure~\ref{fig:ranking}. Note that the general ranking just represents the general opportunity, we cannot promise the evolution-based and surrogate-based definitely outperform \textit{RS} in any scenario. Figure~\ref{fig:ranking} still shows that \textit{RS} is a powerful baseline, which is consistent with our previous conclusion. And evolution-based algorithms shows higher opportunity to be better than \textit{RS}, while surrogate-model-based algorithms have lower opportunity to be better than \textit{RS}, so does other algorithms.

\textbf{10. PBT has the best average ranking among all scenarios}. While no algorithm performs the best in any case, in practice, users still want a recommendation, especially when they have little knowledge about the dataset or the downstream ML model. To give a recommendation, we compute the average rankings of all 15 algorithms under all scenarios (10 datasets $\times$ 6 possitble time budgets $\times$ 3 downstream ML models = 180 scenarios). We rank them in each scenario by validation accuracy (if there is a tie, we select the one with a smaller converge time). Then we rank the average ranking of each algorithm throughout all 180 scenarios, which is shown in Figure~\ref{fig:ranking}. We can see that \textit{PBT} is ranked the top, followed by the other two evolution-based algorithms. \textit{RS}, ranked the fourth, is a strong baseline. %Note that the average ranking just represents the general opportunity, we cannot promise the evolution-based and surrogate-based definitely outperform \textit{RS} in any scenario. Figure~\ref{fig:ranking} still shows that \textit{RS} is a powerful baseline, which is consistent with our previous conclusion. And evolution-based algorithms shows higher opportunity to be better than \textit{RS}, while surrogate-model-based algorithms have lower opportunity to be better than \textit{RS}, so does other algorithms.

\begin{figure}[t]
\centering
\includegraphics[width=\columnwidth]{figures/ranking.pdf}
\vspace{-2em}
\caption{Average ranking of search algorithms. %\jn{Change general ranking to average ranking. remove the background color of the table} \Danrui{Done}
}
\label{fig:ranking}
\end{figure}

% \vspace{-.5em}
\subsection{The Trade-off Between Time and Accuracy}
We explore the trade-off between time and validation accuracy. We select the best four algorithms in Figure~\ref{fig:ranking}, which are \textit{PBT},  \textit{TEVO\_H}, \textit{TEVO\_Y} and \textit{RS}. We vary the time limit from 1 min to 60 mins, and compute the accuracy of these algorithms under different time limits. We have conducted the experiments on all ten datasets with three downstream ML models. We get two main insights. Due to the space constraint, we only show the results of \textit{Australian} and \textit{Madeline} datasets with LR and MLP in Figure~\ref{fig:max_scores_by_time}.

%\begin{figure}[htbp]
%\centering
%\subfigure{
%\label{Fig.sub.1}
%\includegraphics[width=0.45\linewidth]{figures/max_scores_by_time_austrilian_lr.eps}}
%\subfigure{%
%\label{Fig.sub.2}
%\includegraphics[width=0.45\linewidth]{figures/max_scores_by_time_austrilian_mlp.eps}}
%\subfigure{
%\label{Fig.sub.3}
%\includegraphics[width=0.45\linewidth]{figures/max_scores_by_time_madeline_lr.eps}}
%\subfigure{
%\label{Fig.sub.4}
%\includegraphics[width=0.45\linewidth]{figures/max_scores_by_time_madeline_mlp.eps}}
%\caption{The trend of validation accuracy with the increase of time limit (``No FP'' refers to no feature preprocessing). \jn{Change Max Time to Time Limit; Add the acc value for the top line of y-axis}}
%\label{fig:max_scores_by_time}
%\end{figure}

\begin{figure*}[t]
% \vspace{-1em}
\centering
\includegraphics[width=\linewidth]{figures/max_scores_by_time_all_in_one.eps}
% \vspace{-2em}
\caption{The trend of validation accuracy with the increase of time limit (``No FP'' refers to no feature preprocessing).}
\label{fig:max_scores_by_time}
\end{figure*}

\textbf{1. Longer time improves accuracy, especially at starting time.} Figure~\ref{fig:max_scores_by_time} shows that longer time indeed improves validation accuracy. This is because longer search time actually means more evaluated pipelines, i.e. more opportunity of finding a better one. An interesting observation is that the accuracy of all four algorithms have a big jump at  starting time (i.e., under a time limit of $1\sim 5$ mins). At this stage, all algorithms tend to select pipelines randomly. This result implies that random search is a strong baseline at the starting point. Even with randomly chosen pipelines, there is a significant improvement on accuracy compared to ``No FP'' (i.e., no feature preprocessing). When time limit increases, the improvement speed slows down. 

\textbf{2. It is hard to figure out when an algorithm converges. } From Figure~\ref{fig:max_scores_by_time}, we can see that the converge time of an algorithm varies under different datasets and downstream models. For example, \textit{PBT} converges when the time limit is 20 mins on \textit{Australian} dataset with downstream LR model. However, when the downstream model is MLP, it converges at 5 mins. If the dataset is changed to \textit{Madeline}, it needs 30 mins to converge. We can derive similar observations for other algorithms. In summary, it is hard to figure out when an algorithm converges. Different scenarios have their own characteristics, and a fixed time limit cannot fit all.

\subsection{Performance Bottleneck Analysis}
We investigate the performance bottleneck of different algorithms in order to identify the opportunities to enhance their performance. We break down the performance into three parts. (1) ``Pick'': picking up FP pipelines to be evaluated, i.e. picking-up time, which includes \texttt{Step 2} and \texttt{Step 3} in Algorithm~\ref{alg:framework}. (2) ``Prep'': preprocessing training and validation datasets with picked pipelines, i.e. preprocessing time, which is included in \texttt{Step 4} of Algorithm~\ref{alg:framework}. (3) ``Train'': training ML models with preprocessed training dataset, i.e., training time, which is also included in \texttt{Step 4} of Algorithm~\ref{alg:framework}. We conduct experiments on all datasets under different time limits. Due to the space constraint, we only show the results of 10 mins on \textit{Australian} and \textit{Madeline} in Figure~\ref{fig:overhead_aus_made_lr_mlp}. Note that \textit{Hyperband} and \textit{BOHB} are not shown in Figure~\ref{fig:overhead_aus_made_lr_mlp}, because the two methods mix the picking-up and evaluation time, and adopt partial training,  making it impossible to record each part separately as other algorithms. 


%There is still space to help most of search algorithms to overcome \textit{RS}. Fundamentally, \textit{RS} has one biggest advantage which is searching the whole space more exhaustively. Thus the basic idea of improving these algorithms is making them as exhaustive as \textit{RS}. Analysing bottleneck of each algorithm should be the most important thing. In general, there are three subprocesses in all search algorithms have possibility to be bottleneck: (1) picking-up FP pipelines to be evaluated, i.e. picking-up time, which includes \texttt{Step 2} and \texttt{Step 3} in Algorithm \ref{alg:framework} (2) preprocessing training and validation dataset with picked pipelines, i.e. preprocessing time, which is included in \texttt{Step 4} of Algorithm \ref{alg:framework} (3) training ML models with preprocessed training dataset, i.e. training time, which is also included in \texttt{Step 4} of Algorithm~\ref{alg:framework}. We record the time of each part with different time limits. Due to the space, the results of 600 seconds on \textit{Australian} and \textit{Madeline} are drawn in Figure~\ref{fig:overhead}. Note that the bar of \textit{Hyperband} and \textit{BOHB} are not shown in Figure~\ref{fig:overhead}, because the two methods mix the pipeline picking-up and evaluation. Moreover, they have partial training part when evaluating, which makes it impossible to record each part separately as other algorithms. 
%\begin{figure}[tbp]
%\centering
%\subfigure{
%\label{Fig.sub.1}
%\includegraphics[width=0.5\linewidth]{figures/overhead_austrilian_LR_600.eps}}
%\subfigure{
%\label{Fig.sub.4}
%\includegraphics[width=0.45\linewidth]{figures/overhead_madeline_LR_600.eps}}

%\subfigure{
%\label{Fig.sub.2}
%\includegraphics[width=0.5\linewidth]{figures/overhead_austrilian_XGB_600.eps}}
%\subfigure{
%\label{Fig.sub.1}
%\includegraphics[width=0.45\linewidth]{figures/overhead_madeline_XGB_600.eps}}

%\subfigure{
%\label{Fig.sub.3}
%\includegraphics[width=0.5\linewidth]{figures/overhead_austrilian_MLP_600.eps}}
%\subfigure{
%\label{Fig.sub.2}
%\includegraphics[width=0.45\linewidth]{figures/overhead_madeline_MLP_600.eps}}
%\caption{Overhead of each calculating part on \textit{Australian} and \textit{Madeline} with different downstream ML models.}
%\label{fig:overhead_aus_made_lr_mlp}
%\end{figure}

\begin{figure}[t]
% \vspace{-5em}
\centering
\includegraphics[width=\linewidth]{figures/overhead_all_in_one.eps}
\caption{Overhead of each calculating part on \textit{Australian} and \textit{Madeline} with different downstream ML models.}
\label{fig:overhead_aus_made_lr_mlp}
\end{figure}

Different search algorithms have different time distribution, as shown in Figure~\ref{fig:overhead_aus_made_lr_mlp}. For non-surrogate-model-based algorithms,  ``Pick'' is not a bottleneck, and whether ``Prep'' or ``Train'' is a bottleneck depends on datasets and downstream ML models. As for algorithms with surrogate models, longer training of surrogate models are taken, leading to longer ``Pick'' time.  However, whether ``Pick'' is actually a bottleneck depends on datasets and downstream ML models. In the following, we discuss four scenarios in detail. Each scenario has its own bottleneck and requires a different improvement strategy. %Users in reality can figure out their own scenarios with our condition to further improve the algorithms they used.

%\jn{Should we define the scenarios  based on datasets and downstream models only. That is, small/large data + simple/complex model. For each scenario, we discuss what the bottleneck is for different kinds of search algos (e.g., surrogate model based, non-surrogate model based)} \Danrui{Done.} 

%\begin{figure}[h]
%\centering
%\includegraphics[width=\columnwidth]{figures/scenarios.pdf}
%\caption{Different scenarios with  proper improvement strategies. \jn{Make the style of this table consistent with other tables} \Danrui{I think we may do not need to add this table.}}
%\label{fig:scenarios}
%\end{figure}


\emph{Scenario 1: Small Data and Simple Model.} The first scenario has a small dataset and a simple downstream ML model like LR. For this scenario, the bottleneck is determined by the type of the search algorithm. If the search algorithm is with complex surrogate models such as \textit{SMAC}, \textit{PLNE}, and \textit{PLE}, ``Pick'' becomes the bottleneck. This is because the search algorithms with complex surrogate models spend a lot of time for training the surrogate models. And the simple downstream ML model on a small dataset does not take too much  time on ``Prep'' and ``Train''. If the search algorithm is without a surrogate model, ``Prep'' becomes the bottleneck. The reason is that ``Pick'' is short, and the evaluating time is also small, leading to the increase of the number of evaluations, i.e. ``Prep'' becomes the bottleneck. In Figure~\ref{fig:overhead_aus_made_lr_mlp}, \textit{RS, TEVO\_H, TEVO\_Y} and \textit{PBT} 
%(\jn{What are evaluation-based algorithms? It would be better to list them directly}\Danrui{Listed}) 
on \textit{Australian} with LR belong to this situation. 

\emph{Scenario 2: Small Data and Complex Model.} The second scenario has a small dataset and a complex downstream ML model like XGB or MLP. For this scenario, which part becomes bottleneck still depends on the type of search algorithms. If the search algorithm is with complex surrogate models such as \textit{SMAC}, \textit{PLNE} and \textit{PLE}, no matter what the downstream ML model is, ``Pick'' is still the bottleneck. If the search algorithm is with a simple surrogate model or without a surrogate model, ``Train'' is always the bottleneck.

\emph{Scenario 3: Large Data and Simple Model.} The third scenario has a large dataset and a simple  downstream ML model like LR. For this scenario, the bottleneck is ``Prep'' in most cases. This is because the training time of a simple downstream ML model is short even if the dataset is large. However, if the surrogate model of a search algorithm is too complex, like ensemble LSTM, ``Pick'' is still bottleneck. For example, when the dataset is \textit{Madeline} and the downstream ML model is \textit{LR}, the bottleneck of \textit{PLE} is still ``Pick'' because training an ensemble LSTM is too time-consuming.

\emph{Scenario 4: Large Data and Complex Model.} The forth scenario has a large dataset and a complex downstream ML model like XGB or MLP. For this scenario, no matter what the search algorithm is, ``Train'' is always the bottleneck. It is natural that the training process of a complex model on a large dataset takes a lot of time. Also, the time-consuming training process reduces the number of evaluated pipelines, i.e., reduces the time of ``Prep''.

In summary, our bottleneck analysis shows that the bottleneck of a search algorithm depends on which scenario the algorithm will be applied to. Our study can help researchers to develop optimized search algorithms tailored for different scenario. 

%\emph{Scenario 1. } The first scenario requires dataset in small size, the search algorithm should be with complex surrogate model and the downstream ML model is simple. For this scenario, reducing picking-up time is a good improving strategy because picking-up time becomes bottleneck. Only with small datasets, the picking-up time has the opportunity of becoming bottleneck. Otherwise, the preprocessing time or evaluating time will become bottleneck. Search algorithm with complex surrogate models spend lots of time for training. And simple downstream ML model does not take too much training time. Figure~\ref{fig:overhead_aus_made_lr_mlp} illustrates the three requirements. As Figure~\ref{fig:overhead_aus_made_lr_mlp} shows, even with \textit{Australian} dataset, the picking-up time of algorithms without surrogate model or without complex surrogate model cannot be the bottleneck. The picking-up time of algorithms with complex surrogate model like \textit{SMAC} and \textit{PNAS\_LSTM\_NO\_ENSEMBLE} becomes bottleneck, no matter what the downstream ML model is. However, when dataset becomes larger, like \textit{Madeline}, the picking-up time of algorithms with complex surrogate model (except \textit{PNAS\_LSTM\_ENSEMBLE}, because its surrogate model is too complex) is not the bottleneck. 

%\emph{Scenario 2. } The second scenario requires dataset in small size, the search algorithm should be without surrogate model and the downstream ML model is simple. For this scenario, reducing preprocessing time is a good improving strategy because preprocessing time becomes bottleneck. In the first scenario, picking-up time of search algorithms without surrogate model is short, and evaluating time is also small with small dataset and simple downstream model, the side effect of which is the increase of number of evaluations, i.e. preprocessing time becomes bottleneck. Some bars in Figure~\ref{fig:overhead_aus_made_lr_mlp} belongs to the first scenario, like \textit{RS} and evolution-based algorithms on \textit{Australian} with LR. 

%\emph{Scenario 3. } The third scenario requires large size dataset and simple downstream ML model. No requirement for search algorithm. For this scenario, reducing preprocessing time is a good improving strategy because preprocessing time becomes bottleneck. This is because even the dataset is large, the simple downstream model causes short training time. Due to the large dataset, the preprocessing time cannot be neglected and the opportunity of becoming bottleneck is high when downstream model is simple. The results of \textit{Madeline} dataset with LR model in Figure~\ref{fig:overhead_aus_made_lr_mlp} belongs to this scenario. 

%\emph{Scenario 4. } The fourth scenario requires large size dataset and complex downstream ML model like XGB and MLP. No requirement for search algorithm. For this scenario, reducing evaluating time is a good improving strategy. Because complex downstream ML model with large dataset means very long-time training. As Figure~\ref{fig:overhead_aus_made_lr_mlp} shows, when the dataset is \textit{Madeline} with XGB and MLP, the training time becomes bottleneck definitely.

%\begin{itemize}
%    \item Dataset: the input dataset should be small enough, which does not have large number of rows and columns. Search algorithm: the search algorithm should be with complex surrogate model, like RF and LSTM. Downstream ML model: simple model like LR. -> \textbf{reduce picking-up time.}
%    \item Dataset: the input dataset should be with small size. Search algorithm: without surrogate model. Downstream ML model: simple model like LR. -> \textbf{reduce preprocessing time.}
%    \item Dataset: the input dataset should be with large size. Search algorithm: No requirement. Downstream ML model: simple model like LR. -> \textbf{reduce preprocessing time}
%    \item Dataset: the input dataset should be with large size. Search algorithm: No requirement. Downstream ML model: the downstream ML model should be complex, like XGB and MLP. -> \textbf{reduce evaluating time. }
%\end{itemize}


==> src/future-work.tex <==
%\section{Research Opportunity}
%We have discussed the feature preprocessing scenario in detail in the previous section. 

%\textbf{search Feature-specific Feature Preprocessing Workflow.}
%In practice, each feature in one table often has its own feature preprocessing pipeline. With the analysis in Section 1, there are about 1 million pipelines with 7 preprocessors. If a table $T$ has $N$ columns, the size of search space becomes $N^{1M}$, which is too huge to be exhausted. According to our empirical results, one simple idea is to utilize \textit{Evolution}-based algorithms. That is, randomly picking-up some workflows to construct a population and mutating based on this population. \textit{Evoluation}-based algorithms are always efficient. Takeaway of this idea is that the starting population may not be perfect because of the huge search space, which may misdirect following search. Another idea is to consider the search process as a game needing rewards and utilize the self-playing like what have done in AlphaGo \cite{DBLP:journals/nature/SilverSSAHGHBLB17} and Atari \cite{DBLP:journals/corr/MnihKSGAWR13} in \textit{reinforcement learning} area. Though the shortcoming of this idea is non-efficient, with the enough exploring time, \textit{RL} can still generate a promising workflow to users.

%\textbf{Automating Other Data Preparation Stages.}
%In other data preparation stages like data cleaning and feature generation in Figure \ref{}, the proper arrangement of operators is still needed to get best results for downstream applications. For example, for data cleaning stage, there are already a benchmark of investigating the performance of single operator when the downstream application is machine learning \cite{DBLP:conf/icde/LiRBZCZ21}. Also, there are works of automating the generation of data cleaning pipeline for SQL-aggregated queries \cite{DBLP:journals/corr/MnihKSGAWR13}. However, specific dataset with specific downstream task needs specific arrangement. To generate a hybrid solution, one direction is to generalize our scenario into a general framework allowing user to input operators and metrics of downstream applications. Then user can specify the search algorithms and time limitation they want to try and the hybrid way synthesising several search algorithms will select the promising search algorithm with short search time. 

%\textbf{Making search Algorithms Transparent.}  
%Most algorithm mentioned in our work are black-box algorithms. Materials on theoretical explanation for these algorithms are less, which means users cannot monitor the whole search process. Thus, these algorithms are not transparent. To increase the transparency of these search algorithms, theoretical analysis is the most important foundation. Thus the theoretical explanation on different kinds of search spaces (discrete and continuous space, etc.) is a promising and impactful direction to explore. Theoretical explanation can help users to trust the selection of these algorithms and help users to explore how the algorithms find their best pipeline. Utilize these information, users can direct search with their own domain knowledge and make the converge speed faster. 

